Nondeterministic Stacks in Neural Networks

Human language is full of compositional syntactic structures, and although neural networks have contributed to groundbreaking improvements in computer systems that process language, widely-used neural network architectures still exhibit limitations in their ability to process syntax. To address this issue, prior work has proposed adding stack data structures to neural networks, drawing inspiration from theoretical connections between syntax and stacks. However, these methods employ deterministic stacks that are designed to track one parse at a time, whereas syntactic ambiguity, which requires a nondeterministic stack to parse, is extremely common in language. In this dissertation, we remedy this discrepancy by proposing a method of incorporating nondeterministic stacks into neural networks. We develop a differentiable data structure that efficiently simulates a nondeterministic pushdown automaton, representing an exponential number of computations with a dynamic programming algorithm. We incorporate this module into two predominant architectures: recurrent neural networks (RNNs) and transformers. We show that this raises their formal recognition power to arbitrary context-free languages, and also aids training, even on deterministic context-free languages. Empirically, neural networks with nondeterministic stacks learn context-free languages much more effectively than prior stack-augmented models, including a language with theoretically maximal parsing difficulty. We also show that an RNN augmented with a nondeterministic stack is capable of surprisingly powerful behavior, such as learning cross-serial dependencies, a well-known non-context-free pattern. We demonstrate improvements on natural language modeling and provide analysis on a syntactic generalization benchmark. This work represents an important step toward building systems that learn to use syntax in more human-like fashion.

==> figures/01-ns-rnn-cfls/test/dyck.tex <==
% This file was created by tikzplotlib v0.9.2.
\begin{tikzpicture}

\begin{axis}[
title={Dyck},
ymin=-0.02,
ymax=0.12,
]
\path [draw=color0, fill=color0, bars]
(axis cs:40,0.00397435457325653)
--(axis cs:40,-0.0018207756612623)
--(axis cs:42,-0.0076937538589557)
--(axis cs:44,-0.0127886337303192)
--(axis cs:46,-0.0161481346410777)
--(axis cs:48,-0.0164528043966118)
--(axis cs:50,-0.0147326763235661)
--(axis cs:52,-0.0136045899485064)
--(axis cs:54,-0.0145494239396404)
--(axis cs:56,-0.0100510404350069)
--(axis cs:58,-0.0100076372773604)
--(axis cs:60,-0.00988139830351791)
--(axis cs:62,-0.00418288574183191)
--(axis cs:64,0.00203121168041852)
--(axis cs:66,-0.000847079656041668)
--(axis cs:68,0.00190121930370493)
--(axis cs:70,0.00993220718830984)
--(axis cs:72,0.0132089864281447)
--(axis cs:74,0.0138719119687483)
--(axis cs:76,0.018320071886356)
--(axis cs:78,0.0228945518926805)
--(axis cs:80,0.0200687256779975)
--(axis cs:82,0.0259733753481284)
--(axis cs:84,0.0384534015764209)
--(axis cs:86,0.0413594105789218)
--(axis cs:88,0.0506751317012664)
--(axis cs:90,0.0506512339062814)
--(axis cs:92,0.0609880526801557)
--(axis cs:94,0.0768359561303223)
--(axis cs:96,0.0771798420990601)
--(axis cs:98,0.0668813464291176)
--(axis cs:100,0.0877214132540295)
--(axis cs:100,0.109072868500684)
--(axis cs:100,0.109072868500684)
--(axis cs:98,0.0893016981049654)
--(axis cs:96,0.0951347763842185)
--(axis cs:94,0.100337567576246)
--(axis cs:92,0.0803032922156338)
--(axis cs:90,0.0735850274618142)
--(axis cs:88,0.0664746380237882)
--(axis cs:86,0.0675287525854638)
--(axis cs:84,0.0545143693105924)
--(axis cs:82,0.047903616256777)
--(axis cs:80,0.0391361238204906)
--(axis cs:78,0.0441139469417605)
--(axis cs:76,0.0400040249086916)
--(axis cs:74,0.0318763068223729)
--(axis cs:72,0.0335509021064202)
--(axis cs:70,0.0283461919206483)
--(axis cs:68,0.0175162723536913)
--(axis cs:66,0.0151993775044417)
--(axis cs:64,0.0161228341867879)
--(axis cs:62,0.0100328238744378)
--(axis cs:60,0.000393826289150102)
--(axis cs:58,0.00357845242560461)
--(axis cs:56,0.000174427600167019)
--(axis cs:54,-0.00437738751205838)
--(axis cs:52,-0.00366339023878588)
--(axis cs:50,-0.00249206225791725)
--(axis cs:48,-0.00543468673365508)
--(axis cs:46,-0.00275956212975761)
--(axis cs:44,-0.00180220597420127)
--(axis cs:42,0.000429170377621888)
--(axis cs:40,0.00397435457325653)
--cycle;

\path [draw=color1, fill=color1, bars]
(axis cs:40,0.0134687146360565)
--(axis cs:40,0.00601337990093773)
--(axis cs:42,-0.000419198364600862)
--(axis cs:44,-0.00464820037938045)
--(axis cs:46,-0.00949409140329263)
--(axis cs:48,-0.0115684770626649)
--(axis cs:50,-0.0141324472522716)
--(axis cs:52,-0.0153596816690244)
--(axis cs:54,-0.0171431300667384)
--(axis cs:56,-0.0158526806901884)
--(axis cs:58,-0.017473422110998)
--(axis cs:60,-0.0177318764600542)
--(axis cs:62,-0.0164518449421501)
--(axis cs:64,-0.0146945612024745)
--(axis cs:66,-0.013562496633242)
--(axis cs:68,-0.0150918465726973)
--(axis cs:70,-0.0121155309646416)
--(axis cs:72,-0.010040497553915)
--(axis cs:74,-0.00826725757777704)
--(axis cs:76,-0.00433927328046305)
--(axis cs:78,-0.00173633390405762)
--(axis cs:80,0.000417989006801754)
--(axis cs:82,0.00208059444953874)
--(axis cs:84,0.00525602840907601)
--(axis cs:86,0.0114782738333444)
--(axis cs:88,0.0134597494033058)
--(axis cs:90,0.0179566426500777)
--(axis cs:92,0.0216493198613006)
--(axis cs:94,0.0230576608619413)
--(axis cs:96,0.0294636803512422)
--(axis cs:98,0.0292275620913601)
--(axis cs:100,0.0325480545122617)
--(axis cs:100,0.0466848600549522)
--(axis cs:100,0.0466848600549522)
--(axis cs:98,0.0422679425830289)
--(axis cs:96,0.0416636822726614)
--(axis cs:94,0.0337330503446273)
--(axis cs:92,0.0325908828809562)
--(axis cs:90,0.0264425744471846)
--(axis cs:88,0.0221171776370896)
--(axis cs:86,0.0190827863150527)
--(axis cs:84,0.0124994796431158)
--(axis cs:82,0.00775926396176918)
--(axis cs:80,0.00562067396824891)
--(axis cs:78,0.00333049479779356)
--(axis cs:76,-0.000899258419555261)
--(axis cs:74,-0.00486643874934503)
--(axis cs:72,-0.0070453441632563)
--(axis cs:70,-0.0101366223817573)
--(axis cs:68,-0.0132765073581418)
--(axis cs:66,-0.012207423794873)
--(axis cs:64,-0.0129645643170378)
--(axis cs:62,-0.0145560168244375)
--(axis cs:60,-0.0154360015438971)
--(axis cs:58,-0.0154737617978698)
--(axis cs:56,-0.0130301751692051)
--(axis cs:54,-0.0147525941453771)
--(axis cs:52,-0.0121388987286045)
--(axis cs:50,-0.00994018195421175)
--(axis cs:48,-0.00693725951031025)
--(axis cs:46,-0.00439201484444497)
--(axis cs:44,0.00118415843764419)
--(axis cs:42,0.00520500085796941)
--(axis cs:40,0.0134687146360565)
--cycle;

\path [draw=color2, fill=color2, bars]
(axis cs:40,0.0122389907395511)
--(axis cs:40,0.00901278153181818)
--(axis cs:42,0.00263735907887086)
--(axis cs:44,-0.00198155933081797)
--(axis cs:46,-0.00684419645674724)
--(axis cs:48,-0.00993699199128213)
--(axis cs:50,-0.0111671365086461)
--(axis cs:52,-0.0125817398615038)
--(axis cs:54,-0.0155703631520077)
--(axis cs:56,-0.0144120753687733)
--(axis cs:58,-0.0170728204963647)
--(axis cs:60,-0.0171245428070105)
--(axis cs:62,-0.0165650767967294)
--(axis cs:64,-0.0147298588792239)
--(axis cs:66,-0.0136369890884257)
--(axis cs:68,-0.0157706333515687)
--(axis cs:70,-0.0126427471839025)
--(axis cs:72,-0.0106425489497968)
--(axis cs:74,-0.00933388621243551)
--(axis cs:76,-0.00587328000491545)
--(axis cs:78,-0.00294736898470888)
--(axis cs:80,-0.00206291425915856)
--(axis cs:82,-0.000112054685588073)
--(axis cs:84,0.00367121121393739)
--(axis cs:86,0.00901721685772161)
--(axis cs:88,0.0116990076930362)
--(axis cs:90,0.015769938303987)
--(axis cs:92,0.0203872047595101)
--(axis cs:94,0.0213905895143245)
--(axis cs:96,0.0274724256530911)
--(axis cs:98,0.0273555090574962)
--(axis cs:100,0.0314792560290724)
--(axis cs:100,0.0416183460381416)
--(axis cs:100,0.0416183460381416)
--(axis cs:98,0.0370577252087295)
--(axis cs:96,0.0370728650307083)
--(axis cs:94,0.0291428078624567)
--(axis cs:92,0.027575059803399)
--(axis cs:90,0.023682664209942)
--(axis cs:88,0.0185591160803137)
--(axis cs:86,0.0158871163648036)
--(axis cs:84,0.00873947726980204)
--(axis cs:82,0.0053228877539082)
--(axis cs:80,0.0031232325076469)
--(axis cs:78,0.000504220182931917)
--(axis cs:76,-0.00298410963095814)
--(axis cs:74,-0.00675372692211891)
--(axis cs:72,-0.00830055188195785)
--(axis cs:70,-0.0111794117428537)
--(axis cs:68,-0.0147089912594175)
--(axis cs:66,-0.0125354822393105)
--(axis cs:64,-0.0132044131246633)
--(axis cs:62,-0.0144597960585679)
--(axis cs:60,-0.014600301342774)
--(axis cs:58,-0.0142553574857791)
--(axis cs:56,-0.0113659046535666)
--(axis cs:54,-0.0130677836584874)
--(axis cs:52,-0.00995190288588481)
--(axis cs:50,-0.00886393019783711)
--(axis cs:48,-0.00603796251789105)
--(axis cs:46,-0.00259821074207723)
--(axis cs:44,0.0012561981419226)
--(axis cs:42,0.00503560394277143)
--(axis cs:40,0.0122389907395511)
--cycle;

\path [draw=color3, fill=color3, bars]
(axis cs:40,0.00915211050864473)
--(axis cs:40,0.004239334614287)
--(axis cs:42,-0.00468814041089317)
--(axis cs:44,-0.00790152480947355)
--(axis cs:46,-0.0120021856448589)
--(axis cs:48,-0.0134653493469781)
--(axis cs:50,-0.0139095637033049)
--(axis cs:52,-0.0140473561896638)
--(axis cs:54,-0.0165461016088443)
--(axis cs:56,-0.0137834666193513)
--(axis cs:58,-0.016309273171637)
--(axis cs:60,-0.0159510344149431)
--(axis cs:62,-0.0158076687041489)
--(axis cs:64,-0.013921280379241)
--(axis cs:66,-0.0134302790770526)
--(axis cs:68,-0.014959389741883)
--(axis cs:70,-0.0122926303763315)
--(axis cs:72,-0.0104673435982308)
--(axis cs:74,-0.0089669511659228)
--(axis cs:76,-0.00537916060674653)
--(axis cs:78,-0.00280044052962489)
--(axis cs:80,-0.000746712727080017)
--(axis cs:82,0.00101603112057103)
--(axis cs:84,0.00561015280876592)
--(axis cs:86,0.0104847432327164)
--(axis cs:88,0.0140867923249296)
--(axis cs:90,0.018237925710533)
--(axis cs:92,0.0234197638686928)
--(axis cs:94,0.0245607021004629)
--(axis cs:96,0.0322125201290493)
--(axis cs:98,0.0333006534219282)
--(axis cs:100,0.0373451950559627)
--(axis cs:100,0.0572669968550011)
--(axis cs:100,0.0572669968550011)
--(axis cs:98,0.0490800752639405)
--(axis cs:96,0.047037095912823)
--(axis cs:94,0.0367681989332333)
--(axis cs:92,0.0343388661833468)
--(axis cs:90,0.0270645465950624)
--(axis cs:88,0.0222555155748408)
--(axis cs:86,0.01715623606539)
--(axis cs:84,0.00968378995324729)
--(axis cs:82,0.00566936368555402)
--(axis cs:80,0.00272714816306813)
--(axis cs:78,0.000646704788745305)
--(axis cs:76,-0.00233225863439028)
--(axis cs:74,-0.00629512353957754)
--(axis cs:72,-0.00791339286720447)
--(axis cs:70,-0.0100598298897102)
--(axis cs:68,-0.0142510770106474)
--(axis cs:66,-0.0111650734059869)
--(axis cs:64,-0.012096182542615)
--(axis cs:62,-0.0137382789999388)
--(axis cs:60,-0.0137950662452581)
--(axis cs:58,-0.0146849372727912)
--(axis cs:56,-0.0116237509866939)
--(axis cs:54,-0.0143419547791971)
--(axis cs:52,-0.0117735837332055)
--(axis cs:50,-0.0104477334719284)
--(axis cs:48,-0.00842570216740337)
--(axis cs:46,-0.00645168554853076)
--(axis cs:44,-0.00148017515783078)
--(axis cs:42,0.00160331418402354)
--(axis cs:40,0.00915211050864473)
--cycle;

\addplot [line0]
table {%
40 0.00107678945599712
42 -0.0036322917406669
44 -0.00729541985226023
46 -0.00945384838541765
48 -0.0109437455651334
50 -0.00861236929074167
52 -0.00863399009364616
54 -0.00946340572584938
56 -0.00493830641741992
58 -0.00321459242587792
60 -0.0047437860071839
62 0.00292496906630295
64 0.0090770229336032
66 0.00717614892420002
68 0.0097087458286981
70 0.0191391995544791
72 0.0233799442672824
74 0.0228741093955606
76 0.0291620483975238
78 0.0335042494172205
80 0.0296024247492441
82 0.0369384958024527
84 0.0464838854435066
86 0.0544440815821928
88 0.0585748848625273
90 0.0621181306840478
92 0.0706456724478947
94 0.0885867618532842
96 0.0861573092416393
98 0.0780915222670415
100 0.0983971408773569
};
\addlegendentry{LSTM}
\addplot [line1]
table {%
40 0.00974104726849712
42 0.00239290124668428
44 -0.00173202097086813
46 -0.0069430531238688
48 -0.00925286828648757
50 -0.0120363146032417
52 -0.0137492901988144
54 -0.0159478621060578
56 -0.0144414279296968
58 -0.0164735919544339
60 -0.0165839390019756
62 -0.0155039308832938
64 -0.0138295627597562
66 -0.0128849602140575
68 -0.0141841769654196
70 -0.0111260766731994
72 -0.00854292085858563
74 -0.00656684816356103
76 -0.00261926585000916
78 0.00079708044686797
80 0.00301933148752533
82 0.00491992920565396
84 0.0088777540260959
86 0.0152805300741985
88 0.0177884635201977
90 0.0221996085486311
92 0.0271201013711284
94 0.0283953556032843
96 0.0355636813119518
98 0.0357477523371945
100 0.039616457283607
} coordinate[pos=1] (Strat);
\addlegendentry{Strat.}
\addplot [line2]
table {%
40 0.0106258861356846
42 0.00383648151082114
44 -0.000362680594447684
46 -0.00472120359941224
48 -0.00798747725458659
50 -0.0100155333532416
52 -0.0112668213736943
54 -0.0143190734052475
56 -0.01288899001117
58 -0.0156640889910719
60 -0.0158624220748922
62 -0.0155124364276487
64 -0.0139671360019436
66 -0.0130862356638681
68 -0.0152398123054931
70 -0.0119110794633781
72 -0.00947155041587733
74 -0.00804380656727721
76 -0.0044286948179368
78 -0.00122157440088848
80 0.000530159124244167
82 0.00260541653416007
84 0.00620534424186972
86 0.0124521666112626
88 0.015129061886675
90 0.0197263012569645
92 0.0239811322814545
94 0.0252666986883906
96 0.0322726453418997
98 0.0322066171331129
100 0.036548801033607
} coordinate[pos=1] (jm);
\addlegendentry{Sup.}
\addplot [line3]
table {%
40 0.00669572256146587
42 -0.00154241311343482
44 -0.00469084998365217
46 -0.00922693559669485
48 -0.0109455257571907
50 -0.0121786485876166
52 -0.0129104699614346
54 -0.0154440281940207
56 -0.0127036088030226
58 -0.0154971052222141
60 -0.0148730503301006
62 -0.0147729738520439
64 -0.013008731460928
66 -0.0122976762415197
68 -0.0146052333762652
70 -0.0111762301330209
72 -0.00919036823271762
74 -0.00763103735275017
76 -0.0038557096205684
78 -0.00107686787043979
80 0.000990217717994057
82 0.00334269740306252
84 0.00764697138100661
86 0.0138204896490532
88 0.0181711539498852
90 0.0226512361527977
92 0.0288793150260198
94 0.0306644505168481
96 0.0396248080209362
98 0.0411903643429343
100 0.0473060959554819
} coordinate[pos=1] (ours);
\addlegendentry{Ours}
\legend{} % suppress legend
\end{axis}

\end{tikzpicture}


==> figures/01-ns-rnn-cfls/test/marked-reversal.tex <==
% This file was created by tikzplotlib v0.9.2.
\begin{tikzpicture}

\begin{axis}[
title={\MarkedReversal{}},
ymin=-0.02,
ymax=0.3,
]
\path [draw=color0, fill=color0, bars]
(axis cs:41,0.0194466518492119)
--(axis cs:41,-0.000816977529935828)
--(axis cs:43,-0.000768626156918924)
--(axis cs:45,-2.67686374417972e-05)
--(axis cs:47,-0.00236705821367008)
--(axis cs:49,-0.00192022537589498)
--(axis cs:51,0.0014665466484165)
--(axis cs:53,0.00668278136214589)
--(axis cs:55,0.0127382636916889)
--(axis cs:57,0.0218259640135858)
--(axis cs:59,0.0259448712963542)
--(axis cs:61,0.0374055663213408)
--(axis cs:63,0.0498827165997935)
--(axis cs:65,0.0554815259243539)
--(axis cs:67,0.0659826924051326)
--(axis cs:69,0.0751169835781432)
--(axis cs:71,0.0884876439935411)
--(axis cs:73,0.0954606384433024)
--(axis cs:75,0.109658465825182)
--(axis cs:77,0.118081988052704)
--(axis cs:79,0.125739569987985)
--(axis cs:81,0.135945136428749)
--(axis cs:83,0.153394935814441)
--(axis cs:85,0.159615887183495)
--(axis cs:87,0.169400825036114)
--(axis cs:89,0.177204679690069)
--(axis cs:91,0.184065740687101)
--(axis cs:93,0.192133915165529)
--(axis cs:95,0.199668202413858)
--(axis cs:97,0.205383372419119)
--(axis cs:99,0.21418669470891)
--(axis cs:99,0.250576759153981)
--(axis cs:99,0.250576759153981)
--(axis cs:97,0.24001519922826)
--(axis cs:95,0.22215561286552)
--(axis cs:93,0.211970232349639)
--(axis cs:91,0.199789874031641)
--(axis cs:89,0.184637282078477)
--(axis cs:87,0.175664463819005)
--(axis cs:85,0.163452792496097)
--(axis cs:83,0.155208830482369)
--(axis cs:81,0.144029433532732)
--(axis cs:79,0.134222172949516)
--(axis cs:77,0.128992364910702)
--(axis cs:75,0.121671547303014)
--(axis cs:73,0.104868602701178)
--(axis cs:71,0.097479838673422)
--(axis cs:69,0.0834248428146021)
--(axis cs:67,0.075244376032841)
--(axis cs:65,0.0651314569058632)
--(axis cs:63,0.0595204884313015)
--(axis cs:61,0.048896671587741)
--(axis cs:59,0.0437703103532028)
--(axis cs:57,0.0359669334700752)
--(axis cs:55,0.0298432751242393)
--(axis cs:53,0.026858468120091)
--(axis cs:51,0.020994929257043)
--(axis cs:49,0.0209293740420583)
--(axis cs:47,0.0172908649220349)
--(axis cs:45,0.0187134091549556)
--(axis cs:43,0.0184360457797796)
--(axis cs:41,0.0194466518492119)
--cycle;

\path [draw=color1, fill=color1, bars]
(axis cs:41,0.0193567009166357)
--(axis cs:41,-0.000780499348884044)
--(axis cs:43,-0.0114104363990373)
--(axis cs:45,-0.0182197292887715)
--(axis cs:47,-0.0177417049675659)
--(axis cs:49,-0.0168448619304006)
--(axis cs:51,-0.016286789262)
--(axis cs:53,-0.0139519246477533)
--(axis cs:55,-0.0130977919268024)
--(axis cs:57,-0.0129978769013005)
--(axis cs:59,-0.0123825080856555)
--(axis cs:61,-0.0121255313405142)
--(axis cs:63,-0.0133196127383394)
--(axis cs:65,-0.0136237510778479)
--(axis cs:67,-0.0152083475691835)
--(axis cs:69,-0.0155984462910427)
--(axis cs:71,-0.016287598972402)
--(axis cs:73,-0.0153783757291266)
--(axis cs:75,-0.0128844905538978)
--(axis cs:77,-0.00981055767983873)
--(axis cs:79,-0.00579366449298889)
--(axis cs:81,-0.00194134584544955)
--(axis cs:83,0.00221918502965596)
--(axis cs:85,0.0090009153888259)
--(axis cs:87,0.0132457809884857)
--(axis cs:89,0.0198388394734637)
--(axis cs:91,0.0232161346550613)
--(axis cs:93,0.0305060114779472)
--(axis cs:95,0.0355560453732349)
--(axis cs:97,0.0397188013710608)
--(axis cs:99,0.0483550665473422)
--(axis cs:99,0.289764092807972)
--(axis cs:99,0.289764092807972)
--(axis cs:97,0.279573405505056)
--(axis cs:95,0.248987630103511)
--(axis cs:93,0.232853239363834)
--(axis cs:91,0.21763823521478)
--(axis cs:89,0.196225954106879)
--(axis cs:87,0.185383579346519)
--(axis cs:85,0.168127242691502)
--(axis cs:83,0.160669584561582)
--(axis cs:81,0.138475329387178)
--(axis cs:79,0.124159073866407)
--(axis cs:77,0.110298262915972)
--(axis cs:75,0.101887706807094)
--(axis cs:73,0.0916661731664154)
--(axis cs:71,0.0807469252793299)
--(axis cs:69,0.0682433212571576)
--(axis cs:67,0.0608685579148065)
--(axis cs:65,0.0499885217686419)
--(axis cs:63,0.046685615388482)
--(axis cs:61,0.0365760466573828)
--(axis cs:59,0.031257730121865)
--(axis cs:57,0.0230178508652247)
--(axis cs:55,0.0177286915381851)
--(axis cs:53,0.0113877790828202)
--(axis cs:51,0.00909411190459193)
--(axis cs:49,0.00617594737908935)
--(axis cs:47,0.00468108473111681)
--(axis cs:45,0.00459100522295195)
--(axis cs:43,0.00956095921957255)
--(axis cs:41,0.0193567009166357)
--cycle;

\path [draw=color2, fill=color2, bars]
(axis cs:41,0.0190878671219198)
--(axis cs:41,0.00380443105406365)
--(axis cs:43,-0.00661438041323217)
--(axis cs:45,-0.0101865292557058)
--(axis cs:47,-0.00921222926817065)
--(axis cs:49,-0.00948219138090969)
--(axis cs:51,-0.0100869623387586)
--(axis cs:53,-0.0109525937961509)
--(axis cs:55,-0.0112974107912307)
--(axis cs:57,-0.0117384023479034)
--(axis cs:59,-0.0120785224315729)
--(axis cs:61,-0.0128965585983899)
--(axis cs:63,-0.0143642264928673)
--(axis cs:65,-0.014599172505381)
--(axis cs:67,-0.0162648378828156)
--(axis cs:69,-0.0155900785368988)
--(axis cs:71,-0.0157474771194657)
--(axis cs:73,-0.0142529835929606)
--(axis cs:75,-0.0122685408250926)
--(axis cs:77,-0.00884483215269483)
--(axis cs:79,-0.00499164497692336)
--(axis cs:81,-0.000392528907275244)
--(axis cs:83,0.00482227243671599)
--(axis cs:85,0.010640555514449)
--(axis cs:87,0.0180801478132484)
--(axis cs:89,0.0243967643469727)
--(axis cs:91,0.0318884337729505)
--(axis cs:93,0.0385650130795161)
--(axis cs:95,0.0464342007091042)
--(axis cs:97,0.0540782525926733)
--(axis cs:99,0.0610857677143592)
--(axis cs:99,0.205291598711663)
--(axis cs:99,0.205291598711663)
--(axis cs:97,0.195896551335634)
--(axis cs:95,0.191633374849879)
--(axis cs:93,0.181930389475974)
--(axis cs:91,0.169978051910764)
--(axis cs:89,0.162578646333089)
--(axis cs:87,0.149954553308394)
--(axis cs:85,0.147190647143084)
--(axis cs:83,0.135703521815667)
--(axis cs:81,0.121788467503016)
--(axis cs:79,0.112444166197652)
--(axis cs:77,0.102928950741101)
--(axis cs:75,0.0966409367657886)
--(axis cs:73,0.0864373456706603)
--(axis cs:71,0.0794028174008654)
--(axis cs:69,0.0654684510120717)
--(axis cs:67,0.0610775377340356)
--(axis cs:65,0.0497267587009826)
--(axis cs:63,0.0453641577144384)
--(axis cs:61,0.0393392614152586)
--(axis cs:59,0.0334152116287993)
--(axis cs:57,0.0271305151550293)
--(axis cs:55,0.0192341697776134)
--(axis cs:53,0.0181973736439538)
--(axis cs:51,0.014654088902919)
--(axis cs:49,0.0104443255381444)
--(axis cs:47,0.00980166720991308)
--(axis cs:45,0.0145833694259974)
--(axis cs:43,0.0127755772889998)
--(axis cs:41,0.0190878671219198)
--cycle;

\path [draw=color3, fill=color3, bars]
(axis cs:41,0.0121192978733589)
--(axis cs:41,0.000182942185246403)
--(axis cs:43,-0.00994335041423798)
--(axis cs:45,-0.014983980307888)
--(axis cs:47,-0.0141921120814764)
--(axis cs:49,-0.013258154580046)
--(axis cs:51,-0.0120903944548824)
--(axis cs:53,-0.0104931699735299)
--(axis cs:55,-0.00946161607098959)
--(axis cs:57,-0.00807147242790289)
--(axis cs:59,-0.0075108770865417)
--(axis cs:61,-0.00759058541116822)
--(axis cs:63,-0.00744987967017754)
--(axis cs:65,-0.00769422774441207)
--(axis cs:67,-0.00763541110240963)
--(axis cs:69,-0.00761032267621896)
--(axis cs:71,-0.00713491462837997)
--(axis cs:73,-0.00562313788964988)
--(axis cs:75,-0.00327830365186461)
--(axis cs:77,0.000177461162527003)
--(axis cs:79,0.00532952143662427)
--(axis cs:81,0.0110449449652165)
--(axis cs:83,0.0166252103939504)
--(axis cs:85,0.0220831319920724)
--(axis cs:87,0.0271106214799934)
--(axis cs:89,0.0291191672381051)
--(axis cs:91,0.0310170214478608)
--(axis cs:93,0.0321840604222034)
--(axis cs:95,0.0336195038623382)
--(axis cs:97,0.0334337630809231)
--(axis cs:99,0.0203559829036216)
--(axis cs:99,0.330392299715582)
--(axis cs:99,0.330392299715582)
--(axis cs:97,0.234959190815168)
--(axis cs:95,0.199238850890724)
--(axis cs:93,0.166907181767023)
--(axis cs:91,0.131477694404123)
--(axis cs:89,0.0978489247095132)
--(axis cs:87,0.0716374529354706)
--(axis cs:85,0.0486722779264903)
--(axis cs:83,0.0325827892424683)
--(axis cs:81,0.0207867213504315)
--(axis cs:79,0.0114606431780918)
--(axis cs:77,0.00373820673594402)
--(axis cs:75,-0.00205427436577286)
--(axis cs:73,-0.00486612749412289)
--(axis cs:71,-0.00545720052595976)
--(axis cs:69,-0.00551767373447782)
--(axis cs:67,-0.00524932957808678)
--(axis cs:65,-0.00510604062729396)
--(axis cs:63,-0.00541767112710054)
--(axis cs:61,-0.00582823200761881)
--(axis cs:59,-0.00639321430415565)
--(axis cs:57,-0.00686949110817299)
--(axis cs:55,-0.00711566968694599)
--(axis cs:53,-0.00724135810909173)
--(axis cs:51,-0.00763374353365316)
--(axis cs:49,-0.00804103141578053)
--(axis cs:47,-0.00799861952465342)
--(axis cs:45,-0.00699834618848702)
--(axis cs:43,-0.00154961332045941)
--(axis cs:41,0.0121192978733589)
--cycle;

\addplot [line0]
table {%
41 0.00931483715963805
43 0.00883370981143032
45 0.0093433202587569
47 0.00746190335418239
49 0.00950457433308165
51 0.0112307379527298
53 0.0167706247411185
55 0.0212907694079641
57 0.0288964487418305
59 0.0348575908247785
61 0.0431511189545409
63 0.0547016025155475
65 0.0603064914151085
67 0.0706135342189868
69 0.0792709131963726
71 0.0929837413334816
73 0.10016462057224
75 0.115665006564098
77 0.123537176481703
79 0.12998087146875
81 0.139987284980741
83 0.154301883148405
85 0.161534339839796
87 0.17253264442756
89 0.180920980884273
91 0.191927807359371
93 0.202052073757584
95 0.210911907639689
97 0.22269928582369
99 0.232381726931445
};
\addlegendentry{LSTM}
\addplot [line1]
table {%
41 0.00928810078387584
43 -0.000924738589732377
45 -0.00681436203290976
47 -0.00653031011822454
49 -0.0053344572756556
51 -0.00359633867870405
53 -0.00128207278246653
55 0.00231544980569132
57 0.0050099869819621
59 0.00943761101810473
61 0.0122252576584343
63 0.0166830013250713
65 0.018182385345397
67 0.0228301051728115
69 0.0263224374830575
71 0.032229663153464
73 0.0381438987186444
75 0.0445016081265979
77 0.0502438526180667
79 0.0591827046867093
81 0.0682669917708641
83 0.081444384795619
85 0.0885640790401637
87 0.0993146801675021
89 0.108032396790172
91 0.120427184934921
93 0.13167962542089
95 0.142271837738373
97 0.159646103438058
99 0.169059579677657
};
\addlegendentry{Strat.}
\addplot [line2]
table {%
41 0.0114461490879917
43 0.00308059843788381
45 0.00219842008514581
47 0.000294718970871211
49 0.000481067078617348
51 0.00228356328208023
53 0.00362238992390143
55 0.00396837949319135
57 0.00769605640356296
59 0.0106683445986132
61 0.0132213514084343
63 0.0154999656107856
65 0.0175637930978008
67 0.02240634992561
69 0.0249391862375864
71 0.0318276701406999
73 0.0360921810388499
75 0.042186197970348
77 0.0470420592942031
79 0.0537262606103644
81 0.0606979692978703
83 0.0702628971261913
85 0.0789156013287666
87 0.0840173505608211
89 0.0934877053400311
91 0.100933242841857
93 0.110247701277745
95 0.119033787779492
97 0.124987401964154
99 0.133188683213011
};
\addlegendentry{Sup.}
\addplot [line3]
table {%
41 0.00615112002930267
43 -0.0057464818673487
45 -0.0109911632481875
47 -0.0110953658030649
49 -0.0106495929979133
51 -0.00986206899426778
53 -0.00886726404131081
55 -0.00828864287896779
57 -0.00747048176803794
59 -0.00695204569534867
61 -0.00670940870939352
63 -0.00643377539863904
65 -0.00640013418585301
67 -0.0064423703402482
69 -0.00656399820534839
71 -0.00629605757716987
73 -0.00524463269188639
75 -0.00266628900881873
77 0.00195783394923551
79 0.00839508230735806
81 0.015915833157824
83 0.0246039998182093
85 0.0353777049592813
87 0.049374037207732
89 0.0634840459738092
91 0.0812473579259921
93 0.0995456210946134
95 0.116429177376531
97 0.134196476948045
99 0.175374141309602
};
\addlegendentry{Ours}
\legend{} % suppress legend
\end{axis}

\end{tikzpicture}


==> figures/01-ns-rnn-cfls/test/unmarked-reversal.tex <==
% This file was created by tikzplotlib v0.9.2.
\begin{tikzpicture}

\begin{axis}[
title={\UnmarkedReversal{}},
ymax=0.328256274987751,
ymin=0
]
\path [draw=color0, fill=color0, bars]
(axis cs:40,0.181685486959855)
--(axis cs:40,0.144919119716879)
--(axis cs:42,0.132917774978263)
--(axis cs:44,0.127943320726502)
--(axis cs:46,0.121387345219)
--(axis cs:48,0.122128194137432)
--(axis cs:50,0.132533586469534)
--(axis cs:52,0.132479072253934)
--(axis cs:54,0.144345567446157)
--(axis cs:56,0.144524776842252)
--(axis cs:58,0.150252193554495)
--(axis cs:60,0.162091231147468)
--(axis cs:62,0.165384504096011)
--(axis cs:64,0.173169787250933)
--(axis cs:66,0.181898623133316)
--(axis cs:68,0.190448576470662)
--(axis cs:70,0.194177628243421)
--(axis cs:72,0.204372190368375)
--(axis cs:74,0.2071692753159)
--(axis cs:76,0.216394983158359)
--(axis cs:78,0.223277185062583)
--(axis cs:80,0.225172545849746)
--(axis cs:82,0.233323843922851)
--(axis cs:84,0.242654655065135)
--(axis cs:86,0.249554318216498)
--(axis cs:88,0.250486860593374)
--(axis cs:90,0.251551160263491)
--(axis cs:92,0.260102922715376)
--(axis cs:94,0.268237680956334)
--(axis cs:96,0.269947960950872)
--(axis cs:98,0.28047700598532)
--(axis cs:100,0.277905909427444)
--(axis cs:100,0.302969822172908)
--(axis cs:100,0.302969822172908)
--(axis cs:98,0.296636358388712)
--(axis cs:96,0.296435113669178)
--(axis cs:94,0.287988540715421)
--(axis cs:92,0.278940137523913)
--(axis cs:90,0.275860667479671)
--(axis cs:88,0.261295315704974)
--(axis cs:86,0.267222695050937)
--(axis cs:84,0.251826677735393)
--(axis cs:82,0.243407169653237)
--(axis cs:80,0.238575197970366)
--(axis cs:78,0.239088081858623)
--(axis cs:76,0.236144542249192)
--(axis cs:74,0.221648179433678)
--(axis cs:72,0.212098199129384)
--(axis cs:70,0.206497292273842)
--(axis cs:68,0.199506569560822)
--(axis cs:66,0.192706522378211)
--(axis cs:64,0.182363699382943)
--(axis cs:62,0.173709025481618)
--(axis cs:60,0.169939098143082)
--(axis cs:58,0.165617870720124)
--(axis cs:56,0.159483337052572)
--(axis cs:54,0.1645867370419)
--(axis cs:52,0.147282348546067)
--(axis cs:50,0.145870154947365)
--(axis cs:48,0.137591064210792)
--(axis cs:46,0.136827825724417)
--(axis cs:44,0.146046310796615)
--(axis cs:42,0.159087439486309)
--(axis cs:40,0.181685486959855)
--cycle;

\path [draw=color1, fill=color1, bars]
(axis cs:40,0.152577930432876)
--(axis cs:40,0.126020279759483)
--(axis cs:42,0.0991327373623337)
--(axis cs:44,0.083118957823784)
--(axis cs:46,0.0797348273862628)
--(axis cs:48,0.0832355007703479)
--(axis cs:50,0.0869632434116827)
--(axis cs:52,0.0937585417790436)
--(axis cs:54,0.102275146410409)
--(axis cs:56,0.112030364883507)
--(axis cs:58,0.114320023396926)
--(axis cs:60,0.12310501354434)
--(axis cs:62,0.130755810784822)
--(axis cs:64,0.134190948942749)
--(axis cs:66,0.143810713867485)
--(axis cs:68,0.15374463367516)
--(axis cs:70,0.157617805708657)
--(axis cs:72,0.16965631676395)
--(axis cs:74,0.176174527763642)
--(axis cs:76,0.185104297040207)
--(axis cs:78,0.201134559167872)
--(axis cs:80,0.196124788929592)
--(axis cs:82,0.205435463807105)
--(axis cs:84,0.211157919447028)
--(axis cs:86,0.225995451822541)
--(axis cs:88,0.229436585216726)
--(axis cs:90,0.235685741614872)
--(axis cs:92,0.244906748033027)
--(axis cs:94,0.254343848400868)
--(axis cs:96,0.260655246179298)
--(axis cs:98,0.267825172938296)
--(axis cs:100,0.272979582490333)
--(axis cs:100,0.290625895203769)
--(axis cs:100,0.290625895203769)
--(axis cs:98,0.291578509516094)
--(axis cs:96,0.28518044481445)
--(axis cs:94,0.274929663829397)
--(axis cs:92,0.262882469645121)
--(axis cs:90,0.262142817899123)
--(axis cs:88,0.252228270414008)
--(axis cs:86,0.250474898109138)
--(axis cs:84,0.238520330206179)
--(axis cs:82,0.229492124654654)
--(axis cs:80,0.228134795710833)
--(axis cs:78,0.22063064765718)
--(axis cs:76,0.214846566771948)
--(axis cs:74,0.20966259020384)
--(axis cs:72,0.198452283454294)
--(axis cs:70,0.19231968456307)
--(axis cs:68,0.184692661368273)
--(axis cs:66,0.180646216090064)
--(axis cs:64,0.168545159151088)
--(axis cs:62,0.157218688424863)
--(axis cs:60,0.150998704418085)
--(axis cs:58,0.14419970749946)
--(axis cs:56,0.136345058581631)
--(axis cs:54,0.141107570404037)
--(axis cs:52,0.124598619706054)
--(axis cs:50,0.123621513630216)
--(axis cs:48,0.117314832610429)
--(axis cs:46,0.11320023995661)
--(axis cs:44,0.118789019757571)
--(axis cs:42,0.121699509282298)
--(axis cs:40,0.152577930432876)
--cycle;

\path [draw=color2, fill=color2, bars]
(axis cs:40,0.167486612370971)
--(axis cs:40,0.106688428876076)
--(axis cs:42,0.0784022682019458)
--(axis cs:44,0.0643765014745411)
--(axis cs:46,0.0685752212558613)
--(axis cs:48,0.0729738230721517)
--(axis cs:50,0.08407024878105)
--(axis cs:52,0.084605761884122)
--(axis cs:54,0.102920260418912)
--(axis cs:56,0.0960488972132564)
--(axis cs:58,0.108545480032762)
--(axis cs:60,0.119748664649029)
--(axis cs:62,0.125551334940846)
--(axis cs:64,0.137219466129468)
--(axis cs:66,0.14449797161566)
--(axis cs:68,0.152314807587251)
--(axis cs:70,0.162465812787486)
--(axis cs:72,0.174991854188361)
--(axis cs:74,0.178711937560595)
--(axis cs:76,0.194097050883399)
--(axis cs:78,0.202202761137199)
--(axis cs:80,0.200005056509171)
--(axis cs:82,0.212641907404687)
--(axis cs:84,0.218965732447428)
--(axis cs:86,0.221931945888501)
--(axis cs:88,0.236803107454494)
--(axis cs:90,0.241472017064648)
--(axis cs:92,0.248634800011284)
--(axis cs:94,0.25789405297675)
--(axis cs:96,0.263625522582024)
--(axis cs:98,0.272627492573197)
--(axis cs:100,0.274579621954306)
--(axis cs:100,0.313500172146046)
--(axis cs:100,0.313500172146046)
--(axis cs:98,0.306349232770223)
--(axis cs:96,0.295142460078391)
--(axis cs:94,0.293462363176388)
--(axis cs:92,0.28433089949431)
--(axis cs:90,0.276884775956292)
--(axis cs:88,0.268655671294138)
--(axis cs:86,0.268729764871666)
--(axis cs:84,0.259338377510838)
--(axis cs:82,0.24631890800067)
--(axis cs:80,0.238967736139066)
--(axis cs:78,0.241740029822469)
--(axis cs:76,0.235293702936981)
--(axis cs:74,0.217372250719388)
--(axis cs:72,0.210120163998633)
--(axis cs:70,0.205596454269956)
--(axis cs:68,0.198332319142763)
--(axis cs:66,0.18519715081348)
--(axis cs:64,0.174916605343276)
--(axis cs:62,0.168373091814203)
--(axis cs:60,0.163377579355063)
--(axis cs:58,0.155870213282805)
--(axis cs:56,0.14861199639697)
--(axis cs:54,0.150809895631645)
--(axis cs:52,0.135345656662274)
--(axis cs:50,0.132745250448349)
--(axis cs:48,0.128819064019562)
--(axis cs:46,0.131713319252773)
--(axis cs:44,0.13603777937386)
--(axis cs:42,0.146214390645067)
--(axis cs:40,0.167486612370971)
--cycle;

\path [draw=color3, fill=color3, bars]
(axis cs:40,0.241886940895305)
--(axis cs:40,0.155207314218929)
--(axis cs:42,0.11928419536995)
--(axis cs:44,0.124258982328071)
--(axis cs:46,0.0714404717531174)
--(axis cs:48,0.0359677987528458)
--(axis cs:50,0.0183781153119509)
--(axis cs:52,0.023532360306569)
--(axis cs:54,0.0189096909399133)
--(axis cs:56,0.0233046176329023)
--(axis cs:58,0.0281695885521018)
--(axis cs:60,0.0328381089248815)
--(axis cs:62,0.0342148073974884)
--(axis cs:64,0.0445532477903284)
--(axis cs:66,0.0622972554424961)
--(axis cs:68,0.0655070193389973)
--(axis cs:70,0.0872377187264658)
--(axis cs:72,0.0904437098010844)
--(axis cs:74,0.0965077361054431)
--(axis cs:76,0.119622361289043)
--(axis cs:78,0.129525030271045)
--(axis cs:80,0.149484906430495)
--(axis cs:82,0.152355387054733)
--(axis cs:84,0.164903822309356)
--(axis cs:86,0.177077739712524)
--(axis cs:88,0.18101861072821)
--(axis cs:90,0.198021086770059)
--(axis cs:92,0.202831000200942)
--(axis cs:94,0.212658283366708)
--(axis cs:96,0.224953306122384)
--(axis cs:98,0.237091755299386)
--(axis cs:100,0.244782064587142)
--(axis cs:100,0.28842231935696)
--(axis cs:100,0.28842231935696)
--(axis cs:98,0.286601846638422)
--(axis cs:96,0.274737751896103)
--(axis cs:94,0.266837469555046)
--(axis cs:92,0.264278020466337)
--(axis cs:90,0.251554955382825)
--(axis cs:88,0.244297057224967)
--(axis cs:86,0.242351299354329)
--(axis cs:84,0.235811443712899)
--(axis cs:82,0.225778970652453)
--(axis cs:80,0.221720356920867)
--(axis cs:78,0.220757554358495)
--(axis cs:76,0.212590105627553)
--(axis cs:74,0.200377431376398)
--(axis cs:72,0.19860196995275)
--(axis cs:70,0.193070195652404)
--(axis cs:68,0.184377799831274)
--(axis cs:66,0.1759159925785)
--(axis cs:64,0.16861888020097)
--(axis cs:62,0.157250981504737)
--(axis cs:60,0.158893961902127)
--(axis cs:58,0.148990649483293)
--(axis cs:56,0.143374882980673)
--(axis cs:54,0.139307914474069)
--(axis cs:52,0.131234018426125)
--(axis cs:50,0.126125567511198)
--(axis cs:48,0.124101781047202)
--(axis cs:46,0.127499117498723)
--(axis cs:44,0.186371473946466)
--(axis cs:42,0.224021730590158)
--(axis cs:40,0.241886940895305)
--cycle;

\addplot [line0]
table {%
40 0.163302303338367
42 0.146002607232286
44 0.136994815761558
46 0.129107585471708
48 0.129859629174112
50 0.139201870708449
52 0.139880710400001
54 0.154466152244028
56 0.152004056947412
58 0.157935032137309
60 0.166015164645275
62 0.169546764788814
64 0.177766743316938
66 0.187302572755763
68 0.194977573015742
70 0.200337460258631
72 0.208235194748879
74 0.214408727374789
76 0.226269762703775
78 0.231182633460603
80 0.231873871910056
82 0.238365506788044
84 0.247240666400264
86 0.258388506633717
88 0.255891088149174
90 0.263705913871581
92 0.269521530119645
94 0.278113110835877
96 0.283191537310025
98 0.288556682187016
100 0.290437865800176
};
\addlegendentry{LSTM}
\addplot [line1]
table {%
40 0.139299105096179
42 0.110416123322316
44 0.100953988790678
46 0.0964675336714365
48 0.100275166690388
50 0.105292378520949
52 0.109178580742549
54 0.121691358407223
56 0.124187711732569
58 0.129259865448193
60 0.137051858981213
62 0.143987249604843
64 0.151368054046919
66 0.162228464978775
68 0.169218647521716
70 0.174968745135864
72 0.184054300109122
74 0.192918558983741
76 0.199975431906078
78 0.210882603412526
80 0.212129792320212
82 0.21746379423088
84 0.224839124826603
86 0.238235174965839
88 0.240832427815367
90 0.248914279756998
92 0.253894608839074
94 0.264636756115133
96 0.272917845496874
98 0.279701841227195
100 0.281802738847051
} coordinate[pos=1] (Strat);
\addlegendentry{Strat.}
\addplot [line2]
table {%
40 0.137087520623523
42 0.112308329423506
44 0.1002071404242
46 0.100144270254317
48 0.100896443545857
50 0.108407749614699
52 0.109975709273198
54 0.126865078025278
56 0.122330446805113
58 0.132207846657783
60 0.141563122002046
62 0.146962213377524
64 0.156068035736372
66 0.16484756121457
68 0.175323563365007
70 0.184031133528721
72 0.192556009093497
74 0.198042094139991
76 0.21469537691019
78 0.221971395479834
80 0.219486396324119
82 0.229480407702679
84 0.239152054979133
86 0.245330855380084
88 0.252729389374316
90 0.25917839651047
92 0.266482849752797
94 0.275678208076569
96 0.279383991330207
98 0.28948836267171
100 0.294039897050176
} coordinate[pos=1] (jm);
\addlegendentry{Sup.}
\addplot [line3]
table {%
40 0.198547127557117
42 0.171652962980054
44 0.155315228137269
46 0.0994697946259202
48 0.0800347899000236
50 0.0722518414115745
52 0.077383189366347
54 0.0791088027069913
56 0.0833397503067874
58 0.0885801190176973
60 0.0958660354135042
62 0.0957328944511128
64 0.106586063995649
66 0.119106624010498
68 0.124942409585136
70 0.140153957189435
72 0.144522839876917
74 0.14844258374092
76 0.166106233458298
78 0.17514129231477
80 0.185602631675681
82 0.189067178853593
84 0.200357633011127
86 0.209714519533427
88 0.212657833976588
90 0.224788021076442
92 0.233554510333639
94 0.239747876460877
96 0.249845529009244
98 0.261846800968904
100 0.266602191972051
};
\addlegendentry{Ours}
\legend{} % suppress legend
\end{axis}

\end{tikzpicture}


==> figures/07-stack-attention-cfls/test/dyck.tex <==
% This file was created with tikzplotlib v0.9.17.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
\definecolor{color4}{rgb}{0.580392156862745,0.403921568627451,0.741176470588235}
\definecolor{color5}{rgb}{0.549019607843137,0.337254901960784,0.294117647058824}

\begin{axis}[
tick align=outside,
tick pos=left,
title={Dyck},
x grid style={white!69.0196078431373!black},
xmin=37, xmax=103,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={Cross-entropy Diff.},
ymin=0, ymax=0.152653509025148,
ytick style={color=black},
ytick distance=0.1
]
\addplot [cedline, color0]
table {%
40 0.104538189209082
42 0.0872253328976109
44 0.075822695694735
46 0.0681635602403837
48 0.0619428515650126
50 0.0574654756358061
52 0.0580609378103866
54 0.0587534139546345
56 0.0591209304689584
58 0.0610375850428154
60 0.0596186976393801
62 0.0697760361395405
64 0.0652296228598671
66 0.0654627644178406
68 0.071668124052768
70 0.0749635966074638
72 0.0820321965372205
74 0.0814936748444359
76 0.0810624963438599
78 0.0907087653373341
80 0.0829650880978098
82 0.0943354158042414
84 0.0984339077080797
86 0.101233349324993
88 0.101664716637194
90 0.106707079511121
92 0.116283441278066
94 0.147318176216878
96 0.136453732242558
98 0.117956592142523
100 0.145452943792803
};
\addplot [cedline, color1]
table {%
40 0.12063450358378
42 0.0963607609754207
44 0.0849265834322259
46 0.0765387566569417
48 0.0694671457261172
50 0.0625782111911106
52 0.0556716399091195
54 0.0515632310971157
56 0.0482131097519072
58 0.0449314549415966
60 0.0432325817412778
62 0.0424930572439732
64 0.0406115200514804
66 0.0414037279273953
68 0.0411475647849944
70 0.0427121268901951
72 0.0442827109003076
74 0.045800906570853
76 0.0493640901768484
78 0.0512104599849406
80 0.052494348886688
82 0.0562409147690923
84 0.0587986376481958
86 0.0608784627971745
88 0.0640159001867968
90 0.0661889792064554
92 0.0682972632899207
94 0.070832530858948
96 0.0732116500476588
98 0.0744437502659737
100 0.0782269381959217
};
\addplot [cedline, color2]
table {%
40 0.099998671793729
42 0.0875472017252802
44 0.0782379866682716
46 0.0708248375448016
48 0.0649384786258055
50 0.0597391298926526
52 0.0563648886508435
54 0.0525331237563145
56 0.0495275678920499
58 0.0469371725321974
60 0.0439496272964016
62 0.0450882183519166
64 0.0427103701805838
66 0.0438642044048624
68 0.0424212996725437
70 0.0445637066325809
72 0.0442079945498149
74 0.0471274410163492
76 0.0491968538338962
78 0.0518086396629643
80 0.0542895859356761
82 0.0578505559827411
84 0.0622355520561291
86 0.0649217761825636
88 0.0677251580867356
90 0.0725050469103374
92 0.0767079438206375
94 0.0811488751261237
96 0.0839468223001163
98 0.0909966387019037
100 0.096155894386424
};
\addplot [cedline, color3]
table {%
40 0.0989862300453926
42 0.082033839408806
44 0.0760432992321236
46 0.0692228363023396
48 0.0636317035286964
50 0.0619696381452007
52 0.0572271175121339
54 0.0556047277247033
56 0.0552632233329839
58 0.0528058687633943
60 0.053242328866774
62 0.0518437386926753
64 0.0502556453673364
66 0.0478399929799943
68 0.0512669526906024
70 0.0517809937341421
72 0.0512868000125585
74 0.0510638982804322
76 0.0542820800792639
78 0.0568628127097051
80 0.0585908848689494
82 0.0630288967813029
84 0.0695430723522966
86 0.0773080718408601
88 0.0804774874179626
90 0.087174958674094
92 0.0958840762812554
94 0.111455166986564
96 0.111065750489208
98 0.113786319516035
100 0.12713720212074
};
\addplot [cedline, color4]
table {%
40 0.0972237573434404
42 0.0824904423092756
44 0.0767579015081606
46 0.0702258021687601
48 0.0644396498472573
50 0.0613050198751647
52 0.0552825278656606
54 0.0523729579790022
56 0.0502357079153055
58 0.0468904646933829
60 0.0458519018633535
62 0.0446852709184526
64 0.044930387592003
66 0.042467775137239
68 0.0428569665529616
70 0.0430875394479848
72 0.0428232424831768
74 0.0454212361362712
76 0.0472340547347684
78 0.0508319021141925
80 0.055047134922797
82 0.0589834606755451
84 0.0638569371240643
86 0.0674373685477149
88 0.07365808075103
90 0.0778616267878327
92 0.082629461968133
94 0.0870864176230075
96 0.0930005216185196
98 0.0965354104132347
100 0.103425853887793
};
\addplot [cedline, color5]
table {%
40 0.0828802358230181
42 0.0716922357864272
44 0.0683800893327018
46 0.0647825106942398
48 0.061448133988253
50 0.0585548616592956
52 0.0574614853613085
54 0.0535618496610187
56 0.0516422239132402
58 0.0501776752085981
60 0.0484030250531343
62 0.0459862256986479
64 0.0460153515115672
66 0.0456751396283392
68 0.0442237353197368
70 0.0438386612195798
72 0.0443088066833913
74 0.0454322106112357
76 0.0455567410271432
78 0.0477095436077212
80 0.0530720526804278
82 0.0557165621648859
84 0.0629343873894923
86 0.0680199637101067
88 0.0737223809627512
90 0.0789489029972237
92 0.0865978576428916
94 0.0909241910132199
96 0.0998433534296528
98 0.102220349538599
100 0.106541771031281
};
\end{axis}

\end{tikzpicture}


==> figures/07-stack-attention-cfls/test/hardest-cfl.tex <==
% This file was created with tikzplotlib v0.9.17.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
\definecolor{color4}{rgb}{0.580392156862745,0.403921568627451,0.741176470588235}
\definecolor{color5}{rgb}{0.549019607843137,0.337254901960784,0.294117647058824}

\begin{axis}[
tick align=outside,
tick pos=left,
title={Hardest CFL},
x grid style={white!69.0196078431373!black},
xlabel={Length},
xmin=37, xmax=103,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={Cross-entropy Diff.},
ymin=0, ymax=0.451810297151001,
ytick style={color=black}
]
\addplot [cedline, color0]
table {%
40 0.153455758403293
41 0.141411670885438
42 0.137958199608503
43 0.133053502416251
44 0.135397627428215
45 0.120311467925857
46 0.121827011405025
47 0.120374614055784
48 0.117925842495089
49 0.114534212722572
50 0.112910844639801
51 0.109032707213858
52 0.107307234153188
53 0.107391553815837
54 0.106352369030439
55 0.105747338431706
56 0.110186228176485
57 0.101600482198039
58 0.107099356529638
59 0.100071083796303
60 0.102821576182252
61 0.112751019301987
62 0.102427878994464
63 0.105262977567365
64 0.10657976892062
65 0.101197858391302
66 0.105179189217095
67 0.0988987797025653
68 0.108030624732554
69 0.104726554609683
70 0.111580289943145
71 0.110958994873761
72 0.112197135080153
73 0.111723822675983
74 0.11845846734024
75 0.118089768629764
76 0.124434076435141
77 0.11923946068888
78 0.117811327134378
79 0.118348207149107
80 0.123882689747093
81 0.123217188280351
82 0.126151372304465
83 0.128650528792187
84 0.128088391357258
85 0.133471708589819
86 0.132250707217656
87 0.129512382566672
88 0.137020573052523
89 0.136903303167939
90 0.134431201597427
91 0.138609594424462
92 0.139662971067701
93 0.140374859400417
94 0.143986247091968
95 0.148273142951465
96 0.151450225906617
97 0.149901882757807
98 0.151515049119174
99 0.152087120231827
100 0.156540321990242
};
\addplot [cedline, color1]
table {%
40 0.150867599475472
41 0.148459952263157
42 0.139534189431
43 0.130564555979919
44 0.1307670433801
45 0.125445966940432
46 0.118036925802132
47 0.120331155559076
48 0.111818619666341
49 0.108496156978077
50 0.106934551480774
51 0.10146999556416
52 0.105805580475519
53 0.0964121224633205
54 0.100036239645938
55 0.0974058205109638
56 0.102105475734728
57 0.092394140663461
58 0.0966970175415189
59 0.0907121011177596
60 0.0909148628879599
61 0.095001938461919
62 0.0869351107674308
63 0.0893916981788843
64 0.0939524985123565
65 0.0885202526699445
66 0.0878842319604956
67 0.0867832572711267
68 0.0954372282545037
69 0.093584825091299
70 0.0952076596192521
71 0.0942801266180211
72 0.0969986097409694
73 0.0972707914836886
74 0.0998892267916944
75 0.1017250690532
76 0.100067223999006
77 0.0951699001036421
78 0.0995046925585901
79 0.0972754462659726
80 0.101544244041977
81 0.106189441834599
82 0.103924699228501
83 0.102930413672475
84 0.105912353238073
85 0.112268191230397
86 0.108932738240337
87 0.109500757624359
88 0.113681311489736
89 0.115541210806077
90 0.109154516046994
91 0.113769645789273
92 0.115712055195006
93 0.119431959793348
94 0.121939631093651
95 0.130378094747949
96 0.125379541119573
97 0.123534817758814
98 0.127209382144524
99 0.125527274033476
100 0.132439735395115
};
\addplot [cedline, color2]
table {%
40 0.134995053469527
41 0.126593373486598
42 0.120182867945365
43 0.113783143381855
44 0.116926537180962
45 0.103219312845347
46 0.104888577223188
47 0.102203774278977
48 0.0948005973471484
49 0.0938969641060265
50 0.0924900566244382
51 0.0915085228975985
52 0.0864161333250471
53 0.0832003805572998
54 0.0844897170946788
55 0.0899399253225124
56 0.0870061060953011
57 0.0788316183622402
58 0.0792003758348325
59 0.0820602737513747
60 0.0829518421357462
61 0.0826440788541529
62 0.0850909792232826
63 0.080481861672665
64 0.075668210575637
65 0.0797494551918791
66 0.073258853661972
67 0.0816558107573433
68 0.0819741077539842
69 0.0765849687265985
70 0.0817361553488007
71 0.0822049291190206
72 0.0765386160859485
73 0.0793318920514667
74 0.0908143768964194
75 0.0841235726834422
76 0.0852626470871658
77 0.0837693510014432
78 0.0859905469700024
79 0.093969149910597
80 0.0938525768570644
81 0.0953979703920245
82 0.101418332629946
83 0.0949406951737641
84 0.104732784199883
85 0.105195759387024
86 0.109295803110667
87 0.109642969804441
88 0.116134178006198
89 0.11835206985212
90 0.120283157108787
91 0.123942679695835
92 0.128734562881003
93 0.133922179687646
94 0.128501565981485
95 0.138414778983219
96 0.138027970093792
97 0.135719551930342
98 0.140425420508397
99 0.139630833519355
100 0.144751665385661
};
\addplot [cedline, color3]
table {%
40 0.136601314550762
41 0.123746825208084
42 0.126546680226022
43 0.123071169221284
44 0.125543976514892
45 0.121520857624269
46 0.118070125608954
47 0.119581199054008
48 0.113943497644601
49 0.110980142169441
50 0.112993247724178
51 0.109504401535073
52 0.111056980429842
53 0.107315297501307
54 0.108749276243476
55 0.106278530877309
56 0.111649552831478
57 0.103388118644624
58 0.106212428845249
59 0.100981723278062
60 0.101667951834639
61 0.106253337013362
62 0.102441037224739
63 0.0975449137485953
64 0.102293086545752
65 0.0994853223484271
66 0.0994195311945028
67 0.0947075693018256
68 0.102259317226816
69 0.100260974281839
70 0.10021996346273
71 0.0966124019502079
72 0.0962933409489852
73 0.0962279992429926
74 0.0966838313347047
75 0.099265236912385
76 0.0983329950835088
77 0.0956297495292757
78 0.0953613259224519
79 0.0969938085525444
80 0.100662030949011
81 0.122918629246875
82 0.155066571703134
83 0.169913550439848
84 0.188677410742137
85 0.207442529105793
86 0.232585856310979
87 0.252277049434771
88 0.269352564728499
89 0.292280539871324
90 0.300012021312649
91 0.321909564235933
92 0.340284736169681
93 0.370593324044825
94 0.38069368805978
95 0.40608090940656
96 0.414337594159073
97 0.422583765887621
98 0.408107636506977
99 0.420197316465505
100 0.433274581617697
};
\addplot [cedline, color4]
table {%
40 0.154297206048944
41 0.138540478095824
42 0.146878061991484
43 0.135506750138368
44 0.139729280783338
45 0.137451374318431
46 0.128029882240359
47 0.133256197947979
48 0.125308393359475
49 0.122822900052078
50 0.125575911584402
51 0.121632175627252
52 0.121653055176629
53 0.115906411095567
54 0.118102476040783
55 0.116697943185443
56 0.119847871543672
57 0.112610403634406
58 0.111496203584045
59 0.107614129698082
60 0.107070848335909
61 0.112227485934177
62 0.107638566524996
63 0.102036490864986
64 0.108702726146044
65 0.10354515323576
66 0.105600045605328
67 0.10050565592936
68 0.108234750145144
69 0.105564138537609
70 0.107557635079909
71 0.103552615260485
72 0.104122364708192
73 0.101380599666656
74 0.102459405708513
75 0.106552069700347
76 0.106983661943443
77 0.102519953925378
78 0.105173934754778
79 0.10359671045831
80 0.10827496743351
81 0.130662809204533
82 0.166392224042341
83 0.189193462155827
84 0.211153664685271
85 0.214213994465173
86 0.221607246638404
87 0.228194878437026
88 0.246174202111184
89 0.271329864852729
90 0.270870835285943
91 0.285725172782125
92 0.285000750937606
93 0.29110965276379
94 0.294216067918769
95 0.30966463570643
96 0.314444163006028
97 0.321270124329604
98 0.309020326226882
99 0.30733877158987
100 0.322089108159156
};
\addplot [cedline, color5]
table {%
40 0.105331298507878
41 0.0998963852609569
42 0.0973526482743909
43 0.0943136408768639
44 0.0926442901191957
45 0.0899721674444314
46 0.0850843635686911
47 0.081507018077658
48 0.0794240897096801
49 0.0774388154771701
50 0.0758355954231866
51 0.0750076946007421
52 0.0766935903052397
53 0.0708025333311466
54 0.074479607265894
55 0.0726604926326699
56 0.0759783063593702
57 0.071974322897421
58 0.0699706184906461
59 0.066895923352404
60 0.0684356273753333
61 0.0671186551722969
62 0.0660293382800223
63 0.0669646418635894
64 0.065430444506547
65 0.0698902900169267
66 0.0663086339557086
67 0.0671153218017475
68 0.0656783841558743
69 0.0657254915570937
70 0.0657010410991794
71 0.0659099394677356
72 0.0674784494845768
73 0.0672310247048016
74 0.064505344965937
75 0.065021083092808
76 0.0662481382267628
77 0.0657561110546707
78 0.0689834949189612
79 0.0625602709516007
80 0.0670897912863575
81 0.0774458447244419
82 0.0977543201098541
83 0.104227087825749
84 0.114619476414534
85 0.11666280751341
86 0.133674224627656
87 0.137984362849372
};
\end{axis}

\end{tikzpicture}


==> figures/07-stack-attention-cfls/test/marked-reversal.tex <==
% This file was created with tikzplotlib v0.9.17.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
\definecolor{color4}{rgb}{0.580392156862745,0.403921568627451,0.741176470588235}
\definecolor{color5}{rgb}{0.549019607843137,0.337254901960784,0.294117647058824}

\begin{axis}[
tick align=outside,
tick pos=left,
title={\MarkedReversal{}},
x grid style={white!69.0196078431373!black},
xmin=38.1, xmax=101.9,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={Cross-entropy Diff.},
ymin=0, ymax=4.47250564725379,
ytick style={color=black}
]
\addplot [cedline, color0]
table {%
41 0.074606658573548
43 0.0611970466691364
45 0.0559505614065705
47 0.0540338423567549
49 0.0549094171395238
51 0.0570813853178302
53 0.05995449768149
55 0.0647260850262034
57 0.0753304086419711
59 0.0833718183734788
61 0.0904159802095182
63 0.101502484113489
65 0.107145313807425
67 0.12017280991818
69 0.12596169456852
71 0.135151794005092
73 0.139858535202025
75 0.152517707907356
77 0.15707972328034
79 0.167921352036343
81 0.176345906223359
83 0.181943572135121
85 0.186614200601872
87 0.19537953368199
89 0.207761687655148
91 0.20817115345775
93 0.220021204702228
95 0.228901720029245
97 0.242037014100529
99 0.250017926189261
};
\addplot [cedline, color1]
table {%
41 0.101591850588819
43 0.0825557681321606
45 0.0710365482537137
47 0.0635547379738765
49 0.0582812165793863
51 0.0538075544335094
53 0.0503063468427216
55 0.0473017741740341
57 0.0445541414005964
59 0.0440643146479465
61 0.0430024104462566
63 0.0425285942562393
65 0.0424275620262091
67 0.0434416725969309
69 0.0443817023221085
71 0.0453767400026458
73 0.0479434423274752
75 0.0499240094269712
77 0.0525461487743862
79 0.0554391103447931
81 0.0584179948580442
83 0.0612141386979641
85 0.0645148644607054
87 0.0676142977134008
89 0.0710512447391509
91 0.0742090496057594
93 0.0771508845815609
95 0.0805546647756819
97 0.0842532781958677
99 0.0877392110336301
};
\addplot [cedline, color2]
table {%
41 0.0867460744682589
43 0.0740782197851154
45 0.067219027652567
47 0.0623299587379287
49 0.0587865674528911
51 0.0561237581256614
53 0.0536557333987487
55 0.0512982812241133
57 0.0492647914463104
59 0.0475776686144908
61 0.0462441012372201
63 0.0450907724879136
65 0.0440675279204705
67 0.0435449748319263
69 0.0431333113373759
71 0.043218180838193
73 0.0434131157790846
75 0.0441350983801932
77 0.0457965596931345
79 0.0481197888840282
81 0.0509869298916897
83 0.0545717630320026
85 0.0586681127075679
87 0.0628500624250252
89 0.0671796497952806
91 0.0715301722881892
93 0.0759353478879054
95 0.0801920725665016
97 0.0842790286238139
99 0.0885503593658749
};
\addplot [cedline, color3]
table {%
41 0.0723322208951661
43 0.0650144504624603
45 0.0622515869494205
47 0.0597014053907936
49 0.0578873349971611
51 0.0569081391354195
53 0.0559557257922337
55 0.0549331934721033
57 0.0546400636265839
59 0.0534562199909252
61 0.0533169828840279
63 0.0530773558961155
65 0.0533119832306871
67 0.0531094510303122
69 0.0531051665208338
71 0.0533763361457295
73 0.0533495414232715
75 0.0521650985031737
77 0.0517749139063734
79 0.0550138052487611
81 0.0780298254663058
83 0.271503224930799
85 0.670376019094097
87 0.948005128777667
89 1.12017605303945
91 1.21377103779289
93 1.27592206072952
95 1.31814626028278
97 1.330352268463
99 1.34269674212213
};
\addplot [cedline, color4]
table {%
41 0.0735567953082754
43 0.068605560642628
45 0.0647239940920425
47 0.0599396034226093
49 0.05616587230194
51 0.0532361284145308
53 0.0521230270416093
55 0.0505672765159456
57 0.0494422927144976
59 0.0478716461422862
61 0.0459643273678943
63 0.0452474790059222
65 0.0455230752248923
67 0.0460680384217655
69 0.0449480164497654
71 0.0438829934039165
73 0.0438130638807647
75 0.0422434404373853
77 0.041759529632476
79 0.0507622522576539
81 0.0692292817121347
83 0.0924618707034665
85 1.09897677971749
87 2.30007869764262
89 2.89043473716032
91 3.18818065098001
93 3.56601507196917
95 3.86336157236251
97 4.03386286006588
99 4.26129571982171
};
\addplot [cedline, color5]
table {%
41 0.0753982010365726
43 0.068933719081585
45 0.0658695424078188
47 0.0623719819811273
49 0.0598414269235973
51 0.0565620410648192
53 0.0555219974519149
55 0.0541475243842288
57 0.0530869243634833
59 0.05057671571296
61 0.0482523156763631
63 0.047217734137744
65 0.0472648274928292
67 0.0426415546696122
69 0.0385562863631567
71 0.0400807023341472
73 0.0424861854039863
75 0.0408780582243165
77 0.0377847558798524
79 0.0370971711801285
81 0.110574361666959
83 0.110045542455883
85 0.169259789078458
87 0.167951961928386
89 0.168717245618235
91 0.167189664824799
93 0.166119047131904
95 0.161594552024121
97 0.159462002054024
99 0.153365005171606
};
\end{axis}

\end{tikzpicture}


==> figures/07-stack-attention-cfls/test/padded-reversal.tex <==
% This file was created with tikzplotlib v0.9.17.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
\definecolor{color4}{rgb}{0.580392156862745,0.403921568627451,0.741176470588235}
\definecolor{color5}{rgb}{0.549019607843137,0.337254901960784,0.294117647058824}

\begin{axis}[
tick align=outside,
tick pos=left,
title={\PaddedReversal{}},
x grid style={white!69.0196078431373!black},
xmin=37, xmax=103,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={Cross-entropy Diff.},
ymin=0, ymax=0.752206305000722,
ytick style={color=black}
]
\addplot [cedline, color0]
table {%
40 0.188377317441501
41 0.184257858338699
42 0.188191254356599
43 0.162114188148862
44 0.154970003975328
45 0.167343958141887
46 0.1550209938127
47 0.17140059325952
48 0.172610388193784
49 0.127302888544734
50 0.155871518940777
51 0.159415361485156
52 0.152571543431003
53 0.132510608920517
54 0.158598582876882
55 0.140277481311203
56 0.146584792156807
57 0.162594910817864
58 0.144320459251786
59 0.143960991128654
60 0.144743713038394
61 0.158585682059014
62 0.163344119924709
63 0.150868049885453
64 0.170539036376912
65 0.16420362333376
66 0.187517539647629
67 0.159258882169936
68 0.160485588528885
69 0.172723112217741
70 0.195703367399174
71 0.177460679547431
72 0.169608296779017
73 0.201258807549629
74 0.155772405360492
75 0.18371621660654
76 0.208509972891951
77 0.204559635324443
78 0.228398286997051
79 0.204665852683592
80 0.22980900185837
81 0.205306777786512
82 0.197615833043765
83 0.22758274306866
84 0.228586368451069
85 0.227045832885989
86 0.245251641620757
87 0.242554622352554
88 0.265803725790292
89 0.279733577896318
90 0.285438378400954
91 0.284324145410965
92 0.297662146009304
93 0.286795165886795
94 0.324897334251202
95 0.329989507799304
96 0.275857532274829
97 0.312730302605344
98 0.328652653353637
99 0.328527876543602
100 0.346643042342288
};
\addplot [cedline, color1]
table {%
40 0.195310050122237
41 0.186859201488518
42 0.188624268243646
43 0.165716530845573
44 0.15465551322233
45 0.150417107062642
46 0.144971965428634
47 0.162879953757162
48 0.160197691222936
49 0.126015224517669
50 0.151224146739521
51 0.149176860559577
52 0.144102794447022
53 0.132951889892787
54 0.150335977656766
55 0.144626474044865
56 0.151230614695076
57 0.159659843989844
58 0.150582307468234
59 0.147765080588747
60 0.157637567025029
61 0.155907547435801
62 0.148857752398463
63 0.156446362474646
64 0.167708526115879
65 0.162354695942909
66 0.185080805017777
67 0.166569359647081
68 0.166873647858558
69 0.172329330005597
70 0.192862173332305
71 0.188490355963604
72 0.176336970111533
73 0.197253221032501
74 0.163576100283266
75 0.182047200447113
76 0.20988255050833
77 0.207871902816245
78 0.216738891371873
79 0.206790066111114
80 0.222028102688665
81 0.209980631230325
82 0.202052172483838
83 0.246040272926289
84 0.227597555557536
85 0.240107416321509
86 0.239441363542322
87 0.253853222264425
88 0.270070094985206
89 0.286764318506687
90 0.294742472917036
91 0.278685808445395
92 0.308214136417443
93 0.299471660883434
94 0.325112678616699
95 0.340429413654067
96 0.293928613796169
97 0.343026145894781
98 0.367573349207912
99 0.375288103371987
100 0.397494573617346
};
\addplot [cedline, color2]
table {%
40 0.146432969343983
41 0.131101076832133
42 0.115888109564859
43 0.104018444525855
44 0.0947592375987612
45 0.0912505536064751
46 0.0857672822938497
47 0.0810592954534057
48 0.0782842740653197
49 0.0764050313924212
50 0.0719408830210855
51 0.0710958608410504
52 0.0683869037182695
53 0.0653815631813591
54 0.0661773615923612
55 0.0624466305812034
56 0.0622774962816998
57 0.061679339888125
58 0.0617503195167848
59 0.0589210907210438
60 0.0582366297397943
61 0.0589797071003119
62 0.0589361233897742
63 0.0560373139487691
64 0.0561791673981785
65 0.0573522140596401
66 0.0542873276664226
67 0.0549635900409247
68 0.0538522839088509
69 0.0560015653378275
70 0.057411910270124
71 0.0546057232337895
72 0.0552528514636791
73 0.057389316140195
74 0.0556976257910035
75 0.0586058862726546
76 0.0594592982756156
77 0.0616507856891433
78 0.06059049189504
79 0.0633895716821984
80 0.0636991408893841
81 0.064389786048308
82 0.0627610209750915
83 0.0654663318604882
84 0.0668626963959942
85 0.0718196956450946
86 0.0698874141926187
87 0.0754473056127036
88 0.0748449611092512
89 0.0791357028573682
90 0.080201025803253
91 0.0817679701752397
92 0.0802502325522487
93 0.0849660744220075
94 0.0911595130447677
95 0.089003114950044
96 0.0870071492046022
97 0.0915503135754164
98 0.0964346585578869
99 0.0921929421377964
100 0.103234233973037
};
\addplot [cedline, color3]
table {%
40 0.161559667530207
41 0.131529765653099
42 0.130528206065895
43 0.10706624387128
44 0.100971543652976
45 0.105649402391939
46 0.10433048621598
47 0.112756865451425
48 0.115126518924091
49 0.086290302028367
50 0.103015263686345
51 0.10109495679219
52 0.0950912190580296
53 0.0895126078513379
54 0.0950126391299271
55 0.0902491597676928
56 0.0900963993446882
57 0.0949509419430467
58 0.092189699321057
59 0.0855918253210746
60 0.0874420575291862
61 0.0909305975916654
62 0.083991547443241
63 0.0818576808995353
64 0.091285133164744
65 0.0896070432475874
66 0.0960850826549041
67 0.0835846891095435
68 0.0876967996015583
69 0.0894655031334125
70 0.0961792632174989
71 0.0936941461810673
72 0.0810186840752778
73 0.0922964535874725
74 0.0762930258564511
75 0.0863934939815641
76 0.104562245880013
77 0.104547039687272
78 0.110951228306936
79 0.107490127754168
80 0.131810284776787
81 0.126191940366661
82 0.135704694866674
83 0.189592794552871
84 0.2078503037763
85 0.250214478098185
86 0.304095176095119
87 0.340820950632049
88 0.416075546651283
89 0.433177276832608
90 0.441918599451774
91 0.469839089726732
92 0.533012234791598
93 0.559609456819947
94 0.595433534603286
95 0.623142316150535
96 0.572330929693219
97 0.643980165279029
98 0.684215431273938
99 0.689694509796842
100 0.718778201568305
};
\addplot [cedline, color4]
table {%
40 0.159749071085407
41 0.132241681111661
42 0.132279185931321
43 0.105999680375375
44 0.0983517245059862
45 0.103769552572132
46 0.103092821519515
47 0.107041949982553
48 0.110835150424359
49 0.0849361842315606
50 0.101499465811279
51 0.0975620750761731
52 0.0945956631442368
53 0.0913237971305562
54 0.100356346282592
55 0.0924373270288284
56 0.0946473753420114
57 0.0996973367137736
58 0.097262832912574
59 0.0911432460550928
60 0.0893018523991105
61 0.0955890644484561
62 0.0843807524207707
63 0.0864554525702955
64 0.0994160538604494
65 0.0921288028292203
66 0.103054437149343
67 0.0894817563237326
68 0.0930564846969364
69 0.0944641173306257
70 0.109483720975134
71 0.09941494501981
72 0.087344979994694
73 0.104549062913131
74 0.0814181143970686
75 0.0945489114974651
76 0.118514805590557
77 0.123797354910977
78 0.131635466382506
79 0.11646112449343
80 0.139883241505362
81 0.133470074684602
82 0.147867585249705
83 0.202606328084815
84 0.195468946204704
85 0.236133543699197
86 0.271858971770518
87 0.304315625929745
88 0.341816410314024
89 0.351999816809382
90 0.365414454435056
91 0.374338020893904
92 0.417461437387691
93 0.429842190085035
94 0.46599283183555
95 0.478679738899806
96 0.409191503195866
97 0.470651262267407
98 0.497258375077676
99 0.51294917595224
100 0.527459348609793
};
\addplot [cedline, color5]
table {%
40 0.118727664341969
41 0.104556881889453
42 0.0917655978189894
43 0.0870833612574233
44 0.0829463271351543
45 0.0807323384755625
46 0.0772942739828137
47 0.0769697494207435
48 0.0751094418522375
49 0.0733468189013022
50 0.0717058644413799
51 0.0708032044007443
52 0.0691011044390219
53 0.0681334481961607
54 0.066257970645851
55 0.0662406838954441
56 0.0636620885853239
57 0.0647596902417961
58 0.0627585991942886
59 0.060693447471386
60 0.0601517505819559
61 0.0605621070407008
62 0.0592134017685317
63 0.0577070566149383
64 0.0573561707933875
65 0.0567934002007807
66 0.0561579577909672
67 0.0549110747523666
68 0.0553067225520165
69 0.0558860345070863
70 0.0543421290580592
71 0.0534750375628401
72 0.052896245853346
73 0.0513569748967194
74 0.0505661083019791
75 0.0506544848085084
76 0.0502161329199654
77 0.0523721161393812
78 0.0556253884739755
79 0.0588819341762689
80 0.0597423633199263
81 0.0674576441347939
82 0.0727387821499549
83 0.076120036998045
84 0.0834250427398314
85 0.0906536792097427
86 0.0926896290010631
87 0.0992908628140585
88 0.115204735526705
89 0.121602565352068
90 0.11813988119535
91 0.132607901033549
92 0.1371817348342
};
\end{axis}

\end{tikzpicture}


==> figures/07-stack-attention-cfls/test/unmarked-reversal.tex <==
% This file was created with tikzplotlib v0.9.17.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
\definecolor{color4}{rgb}{0.580392156862745,0.403921568627451,0.741176470588235}
\definecolor{color5}{rgb}{0.549019607843137,0.337254901960784,0.294117647058824}

\begin{axis}[
tick align=outside,
tick pos=left,
title={\UnmarkedReversal{}},
x grid style={white!69.0196078431373!black},
xmin=37, xmax=103,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={Cross-entropy Diff.},
ymin=0, ymax=1.01305569732219,
ytick style={color=black}
]
\addplot [cedline, color0]
table {%
40 0.294104164887813
42 0.227023082709031
44 0.216680429107512
46 0.220153400173459
48 0.214415356863473
50 0.218886901752492
52 0.217807823401116
54 0.226821062255073
56 0.23332673537579
58 0.237831985179616
60 0.238318554167256
62 0.237723153981616
64 0.252931481802003
66 0.256478600156095
68 0.264440223363436
70 0.264244822347894
72 0.277224150409552
74 0.271805120947197
76 0.286450635574299
78 0.302081749859658
80 0.309239378336312
82 0.308494814865175
84 0.320323423224512
86 0.328448018247192
88 0.316752722454535
90 0.332064780977645
92 0.343530856786106
94 0.363486710987549
96 0.348468965377357
98 0.369955009564413
100 0.38996520030135
};
\addplot [cedline, color1]
table {%
40 0.239283058689269
42 0.217366212460984
44 0.209140723273707
46 0.206493949787445
48 0.212509197491154
50 0.2102769819637
52 0.219685267098365
54 0.230967624286426
56 0.234909356511143
58 0.235166875296721
60 0.243861873665269
62 0.243774503127139
64 0.247189862474752
66 0.256624465692782
68 0.261317883085104
70 0.269045048939388
72 0.276201868914415
74 0.27789529067948
76 0.290843762538401
78 0.294149015779079
80 0.307590075734946
82 0.314738389296085
84 0.312048889937321
86 0.322999621565829
88 0.326249069801059
90 0.343395682122521
92 0.334837166030802
94 0.344595289728589
96 0.351900926843387
98 0.353710987275232
100 0.374461248213573
};
\addplot [cedline, color2]
table {%
40 0.103821391686008
42 0.0847217717995029
44 0.0745856613993899
46 0.067007504576914
48 0.0641658709404859
50 0.0592823984099904
52 0.0559292504677334
54 0.0534793618078254
56 0.0523006122592491
58 0.0510486804983696
60 0.0482935643894678
62 0.0479254543273275
64 0.046738817220089
66 0.0447814912239274
68 0.0450093634997459
70 0.0455627681100779
72 0.0445491439545073
74 0.0454199394216005
76 0.0478147743964658
78 0.0526228180113841
80 0.0537942867119477
82 0.0644258808533298
84 0.0665469096933879
86 0.070586210263345
88 0.0865186692608172
90 0.0880229587513156
92 0.115776348278538
94 0.124931841602598
96 0.117992377299913
98 0.143806585161992
100 0.160981104290578
};
\addplot [cedline, color3]
table {%
40 0.171727865044271
42 0.133085067735229
44 0.130598681666843
46 0.139046596834402
48 0.151760304388515
50 0.161694988758394
52 0.153453461895549
54 0.165881128059123
56 0.170405416056952
58 0.164498507719901
60 0.170570276403135
62 0.160815935347326
64 0.174050136146936
66 0.1721749851874
68 0.168205079034907
70 0.177782099591461
72 0.17614544087404
74 0.185998435518629
76 0.184187757577815
78 0.203594288495081
80 0.225374097301206
82 0.396377525670896
84 0.591160005784841
86 0.647204239843034
88 0.649863401489476
90 0.702553841387486
92 0.716901752870309
94 0.871201021804896
96 0.966936337638017
98 0.958873342860003
100 0.96518918188112
};
\addplot [cedline, color4]
table {%
40 0.185749240899765
42 0.149008407254401
44 0.13913502793369
46 0.140359056880733
48 0.141860504208074
50 0.143576052577314
52 0.138155653830609
54 0.141767646098225
56 0.137951167584677
58 0.138142893956431
60 0.142572223255851
62 0.131416476033451
64 0.138541296898028
66 0.152559867455396
68 0.138739020163436
70 0.144396749277176
72 0.142700730554222
74 0.154098348221415
76 0.16347981112801
78 0.173586342296757
80 0.193935008581916
82 0.248276609233002
84 0.339571620154453
86 0.477819925051765
88 0.545296154858418
90 0.614769453646996
92 0.653349871524547
94 0.6820305276913
96 0.692567768472712
98 0.727039274925795
100 0.731439009475201
};
\addplot [cedline, color5]
table {%
40 0.120885588419395
42 0.0850090394288991
44 0.0707714395722455
46 0.0648806046785769
48 0.0632481949165394
50 0.0709174721536085
52 0.0690132114454134
54 0.0754206642646195
56 0.0775438388765007
58 0.0802647467370142
60 0.0816436756409582
62 0.0768271051993675
64 0.0745977682579447
66 0.0785415095226967
68 0.0758881312886135
70 0.0794490016881559
72 0.0857906444052911
74 0.0879779252473275
76 0.09779513497146
78 0.112045331744825
80 0.132719718112153
82 0.142915169065181
84 0.173425553153903
86 0.195864532069175
88 0.208669614459306
90 0.2468943604447
92 0.259407158645751
94 0.275315217027466
96 0.349517546734992
98 0.357397067167702
100 0.381797447957381
};
\end{axis}

\end{tikzpicture}


==> figures/07-stack-attention-cfls/train/dyck.tex <==
% This file was created with tikzplotlib v0.9.17.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
\definecolor{color4}{rgb}{0.580392156862745,0.403921568627451,0.741176470588235}
\definecolor{color5}{rgb}{0.549019607843137,0.337254901960784,0.294117647058824}

\begin{axis}[
tick align=outside,
tick pos=left,
title={Dyck},
x grid style={white!69.0196078431373!black},
xmin=-4.35, xmax=113.35,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={Cross-entropy Diff.},
ymin=0, ymax=0.286489333291584,
ytick style={color=black}
]
\addplot [cedline, color0]
table {%
1 0.253709071823579
2 0.141509801962839
3 0.118360686129029
4 0.103769605300618
5 0.0835974742506944
6 0.076160837674856
7 0.0848154312898841
8 0.0629980574093579
9 0.0623040018366003
10 0.0644110679212991
11 0.0564781907141091
12 0.0590169113179899
13 0.058946098627441
14 0.0530215365919038
15 0.0533222220712928
16 0.0494193915287051
17 0.0441459971999132
18 0.0414692726342056
19 0.0409585145676405
20 0.0442368418272316
21 0.0337648003947811
22 0.0335469798163066
23 0.0416935316773331
24 0.0452739770057122
25 0.0305501134505483
26 0.0387043820409637
27 0.0379699504717946
28 0.0346202666636771
29 0.0352617074506436
30 0.036935587182605
31 0.0384657137387535
32 0.0407795148296453
33 0.0324786670860604
34 0.0349104178720739
35 0.0294090552498052
36 0.0315505942884867
37 0.0309939263713435
38 0.0279783395803437
39 0.0474660993023014
40 0.0421134704238396
41 0.0239847576999449
42 0.0319180423043974
43 0.0256936433270093
44 0.0256128828984333
45 0.0255930405180025
46 0.026403107547506
47 0.0323099098412368
48 0.0274058223714071
49 0.029389191531881
50 0.0203567029648077
51 0.0235421183413004
52 0.0300348680594471
53 0.0242494249938348
54 0.022502744214649
55 0.028744486604607
56 0.0228147519636326
57 0.0214022734003705
58 0.0373716655100631
59 0.0269453771224233
60 0.0290976856407478
};
\addplot [cedline, color1]
table {%
1 0.260320236539921
2 0.0198157017842102
3 0.00865847522171004
4 0.0147528038975508
5 0.00582333034725369
6 0.00409154687662738
7 0.00456805911121638
8 0.00426680864479123
9 0.00557509761495678
10 0.00403453899143147
11 0.0103577440589451
12 0.00235755748894428
13 0.00275474827213273
14 0.00636735047384884
15 0.00332484791128307
16 0.00259202909989553
17 0.00327606779479861
18 0.00337784733288438
19 0.00176934478124657
20 0.0021753443846666
21 0.00470162325629508
22 0.00630043056242702
23 0.0034855903205131
24 0.00674857966289977
25 0.00176549172666163
26 0.00138462878814316
27 0.00153964432587628
28 0.00245898364475972
29 0.00413680405893879
30 0.00271406031267651
31 0.00182301236260252
32 0.00528168144538776
33 0.00224951803635776
34 0.00188223210405258
35 0.00158694211757182
36 0.00158484459087549
};
\addplot [cedline, color2]
table {%
1 0.170700265838205
2 0.0173951459373185
3 0.00776949863972987
4 0.00669247834998321
5 0.00552131338762074
6 0.00439265139859091
7 0.00757355733521159
8 0.00399171380391927
9 0.00704564435164801
10 0.00621981291362039
11 0.00875861767396957
12 0.00334721073479183
13 0.00549583978449331
14 0.00482684543125822
15 0.00321714297152742
16 0.00588007996158402
17 0.00737885157641338
18 0.00591825100331267
19 0.00528336102143823
20 0.00585598882580629
21 0.00601256265511863
22 0.00227793868062154
23 0.00304829842821075
24 0.00370994068268704
25 0.00270610641927116
26 0.00222846670793309
27 0.00269970555031362
28 0.0053533493712048
29 0.00256100050010866
30 0.00251975313005592
31 0.00255064227448709
32 0.00260119685399707
33 0.00384604376587105
34 0.00216477492781042
35 0.00236736431071782
36 0.00478604333904609
37 0.00319386216118911
38 0.00285354302695051
39 0.00271882892982311
40 0.00384122192835445
41 0.00247020544007726
42 0.00218185444191665
43 0.002886695165632
44 0.00423577018716559
};
\addplot [cedline, color3]
table {%
1 0.272912918791421
2 0.194966962473404
3 0.157607408640165
4 0.126985376531694
5 0.120126484922552
6 0.0977066014473145
7 0.0947968262926883
8 0.0710771121503782
9 0.0673598642643715
10 0.0767934522065701
11 0.0583414634771207
12 0.0688494904548175
13 0.0624021047096165
14 0.0577549591682117
15 0.050562656859794
16 0.0366681821985572
17 0.0634968293951759
18 0.0398312475889216
19 0.0352947487544234
20 0.0736787750522899
21 0.0484445613364582
22 0.0421003766271798
23 0.0337868735339938
24 0.0327895127436169
25 0.0331338807184453
26 0.0477295741432688
27 0.0239608939124616
28 0.030555222132744
29 0.0286996107213502
30 0.0336289397957451
31 0.0229123120311095
32 0.0214534410805536
33 0.0291943217196241
34 0.0222756150934192
35 0.037535483098148
36 0.02835695723702
37 0.0226393583371393
38 0.0320304462434906
39 0.0253826363852655
40 0.0185525900329044
41 0.0176789692656102
42 0.0219886075809139
43 0.0287729467197597
44 0.0295175875408419
45 0.0384851009147926
46 0.0160944123349956
47 0.0182916726921795
48 0.0305754596483225
49 0.0186956033136049
50 0.0171072661178169
51 0.0385088498874643
52 0.0217932180841632
53 0.0202649473521926
54 0.0176733463950528
55 0.0155721638333041
56 0.0151080139979236
57 0.0280865292120275
58 0.017289510745108
59 0.0181570319147405
60 0.014105946562644
61 0.0157559794660382
62 0.0156322656377966
63 0.0131131120965328
64 0.0165171751384008
65 0.0136979228111771
66 0.0217613688939262
67 0.0138350467715695
68 0.0156597328379704
69 0.0182396917925727
70 0.0108060649335235
71 0.0382361043010075
72 0.0156616109095712
73 0.0152482327370373
74 0.0146219110921862
75 0.0120508491719579
76 0.0169303808903726
77 0.0102881272906025
78 0.0138894912937026
79 0.0107897876055999
80 0.011523537447286
81 0.0140764380377054
82 0.0102468223080592
83 0.0117106912927712
84 0.012074056282759
85 0.0127974475034281
86 0.0137744840474139
87 0.0156070280153084
88 0.0110801447776222
89 0.00854629118077643
90 0.012739294088582
91 0.0108456955806159
92 0.0145056953879531
93 0.0104384630210158
94 0.0100663585321905
95 0.0142004620322165
96 0.0158366082296011
97 0.0127553042729431
98 0.00822102184786833
99 0.0122493291458329
100 0.0169480825440064
101 0.0157611436573944
102 0.00968797525139031
103 0.0146590408666272
104 0.0113216124399913
105 0.00973024794474819
106 0.00880302670724387
107 0.0114396132656625
108 0.008849591375235
};
\addplot [cedline, color4]
table {%
1 0.0163534581291562
2 0.0108425868085205
3 0.00984889341189676
4 0.00450868191451426
5 0.00454826218065452
6 0.00387958517784515
7 0.00353127754731475
8 0.00421065044757996
9 0.00383795642802542
10 0.00886841309912167
11 0.00338658953653437
12 0.00345025008092248
13 0.00503236964580367
14 0.00613920842359017
15 0.0075891148463586
16 0.00243262404016653
17 0.00327710772099754
18 0.00303406285564733
19 0.0088263997657404
20 0.00393477033476464
21 0.00627163354544635
22 0.00344596650791329
23 0.00348059153111169
24 0.00339325326005646
25 0.00360028254758715
26 0.00306810697707005
};
\addplot [cedline, color5]
table {%
1 0.00770236341542885
2 0.00599471506334004
3 0.00456187270927488
4 0.00387391297883233
5 0.00481878203665742
6 0.00428098516121345
7 0.00744024954821765
8 0.00345551466493854
9 0.00465349736621978
10 0.00223153629149231
11 0.00422922312606655
12 0.00277031674253636
13 0.00213108397212303
14 0.00322111840687578
15 0.00992311449288352
16 0.00211291662154078
17 0.00186224520455147
18 0.00191311375213599
19 0.00190821231261307
20 0.00186684798806991
21 0.00196678892019309
22 0.00191323329914128
23 0.0021266019261682
24 0.00482807960534326
25 0.00179314112870455
26 0.00203689702207366
27 0.00222012312144082
28 0.00138882245934013
29 0.00224121646975584
30 0.00372774407449694
31 0.00250618989704066
32 0.00275598329017535
33 0.00174507630862242
34 0.00347729813232012
35 0.00226583477253306
36 0.00155231556219693
37 0.00288414094935341
38 0.00398737304754182
};
\end{axis}

\end{tikzpicture}


==> figures/07-stack-attention-cfls/train/hardest-cfl.tex <==
% This file was created with tikzplotlib v0.9.17.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
\definecolor{color4}{rgb}{0.580392156862745,0.403921568627451,0.741176470588235}
\definecolor{color5}{rgb}{0.549019607843137,0.337254901960784,0.294117647058824}

\begin{axis}[
tick align=outside,
tick pos=left,
title={Hardest CFL},
x grid style={white!69.0196078431373!black},
xlabel={Epoch},
xmin=-8.7, xmax=204.7,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={Cross-entropy Diff.},
ymin=0, ymax=0.171681568044367,
ytick style={color=black}
]
\addplot [cedline, color0]
table {%
1 0.157914707886522
2 0.125183848644569
3 0.111740959423211
4 0.107639005059214
5 0.094962631959453
6 0.0953033135292305
7 0.0874006525876727
8 0.0885720473723766
9 0.0838141937526424
10 0.0819879380998225
11 0.0828928237894566
12 0.0796460736204874
13 0.0845095257522939
14 0.077495675761075
15 0.0752765530641128
16 0.0743155591024356
17 0.0815581953023035
18 0.0742642488256453
19 0.0805575243313557
20 0.0719533436809303
21 0.0703218839328674
22 0.0705961149314758
23 0.0708469338752584
24 0.0701994446237655
25 0.0684565510201833
26 0.070324717411
27 0.073189744233207
28 0.0727140743515786
29 0.0695723364578271
30 0.0672707923931053
31 0.0656438707835334
32 0.0655402419857163
33 0.0638028947648615
34 0.0672942387490236
35 0.0619119316600314
36 0.0619805078595135
37 0.0607181091579159
38 0.0612452119687263
39 0.0601940258826796
40 0.063051261159736
41 0.0615305118259672
42 0.0624617553066809
43 0.058932344385745
44 0.0573183158292747
45 0.0602946153958086
46 0.0583020150353852
47 0.058552380788975
48 0.057045749992797
49 0.0608222348018619
50 0.0569647879806126
51 0.060414149506312
52 0.0562823770985932
53 0.0579416914126845
54 0.0566336888887893
55 0.0548950694092278
56 0.0555590439736995
57 0.0555408945380169
58 0.0560852092213127
59 0.0562248229835263
60 0.0562850567415225
61 0.0593710751089469
62 0.0541799934928024
63 0.06127730739711
64 0.0546171058280907
65 0.055522737826345
66 0.0537139746913133
67 0.055550061245152
68 0.0531438396007218
69 0.0541617006161872
70 0.0563680227690551
71 0.0534958259790719
72 0.0542234727262141
73 0.0556537669605706
74 0.0531193943554105
75 0.0519668298311056
76 0.0516118519817117
77 0.0524172478720333
78 0.0522389403985362
79 0.0520581112750209
80 0.0534188647215947
81 0.0520935131208438
82 0.0520133369155076
83 0.0508344218761125
84 0.0523912798660968
85 0.0512125197013318
86 0.0512247495999767
87 0.0527172982385102
88 0.0526875384027032
89 0.050948965697359
90 0.0516721834458502
91 0.0507769186929712
92 0.0506289708046876
93 0.0511184047792839
94 0.0502153588755245
95 0.0523065509702909
96 0.0511831361381159
97 0.0527822582712929
98 0.0509759564995107
99 0.0504558687818462
100 0.0504699062441276
101 0.0506306827410354
102 0.0511589382764419
103 0.0513009822190935
104 0.0497029088678078
105 0.0515240287115843
106 0.0500255148012232
107 0.0547886383160898
108 0.0514091034206112
109 0.0502501173160046
110 0.0494794310130919
111 0.0503550911324215
112 0.0530830060933192
113 0.0507695741014509
114 0.0519541436239863
115 0.0516864402272386
116 0.0497244114951467
117 0.0500755798444101
118 0.0504014173565173
119 0.05081749064893
120 0.0498485668983046
};
\addplot [cedline, color1]
table {%
1 0.127536964671586
2 0.105191353476081
3 0.0961654462619006
4 0.097246840766757
5 0.088715844764244
6 0.0778697559589674
7 0.0768021671706349
8 0.0715988590040699
9 0.0692600140148749
10 0.0658476365902498
11 0.0655131906126967
12 0.0664837554972426
13 0.0631727387920609
14 0.0632205791943121
15 0.064780390959202
16 0.0623599234132055
17 0.0652630910665359
18 0.0592329520407915
19 0.0615660987861697
20 0.0648140947068951
21 0.0586518228158635
22 0.057918596506872
23 0.0589259362440702
24 0.0620850411904881
25 0.0572829979362963
26 0.0646283885743302
27 0.0583459036968745
28 0.0587961117988567
29 0.0553347881298101
30 0.0579371127444639
31 0.0558828602090509
32 0.0541604998278362
33 0.0541907007237192
34 0.0529143195655428
35 0.0519155984730311
36 0.0536651517779636
37 0.0510019406746076
38 0.0520662200825963
39 0.0486603819935307
40 0.0509167602793685
41 0.0525558026827746
42 0.0489507663720499
43 0.0507509185750341
44 0.0494205354575414
45 0.048753503883324
46 0.0463557743259673
47 0.0460338021666333
48 0.0459155503699149
49 0.0495571212213652
50 0.0444661130582542
51 0.0460702308071881
52 0.044683870284882
53 0.0448110696277795
54 0.0477314379127312
55 0.0441677189610319
56 0.0471747879196391
57 0.0436094865750001
58 0.0477423293380106
59 0.0445854472769129
60 0.0443563251290489
61 0.0461619780313001
62 0.0464623322999569
63 0.0445480451694018
64 0.0427038293308419
65 0.0431707615136758
66 0.0433194382258697
67 0.0428569569050308
68 0.0436661177097155
69 0.0439308263881206
70 0.0422440688297809
71 0.0429218217780416
72 0.0417872246565061
73 0.04198948889177
74 0.0449332539866174
75 0.0413653305944752
76 0.0434054851696233
77 0.0458251554095248
78 0.0459856705389119
79 0.0437624104950138
80 0.043182909485215
81 0.0410589715824685
82 0.0425053958306099
83 0.0427381460776017
84 0.0443855515397045
85 0.0491533340520345
86 0.0427597568403828
87 0.0408945391650251
88 0.0418043346620194
89 0.041086649203123
90 0.0410720746920885
91 0.0434746430726436
92 0.0425021648571233
93 0.0410477105248614
94 0.0439529411949846
95 0.042478837289647
96 0.0413373729493303
97 0.0428326263407424
};
\addplot [cedline, color2]
table {%
1 0.164026004192887
2 0.130619238569181
3 0.121611081497613
4 0.102869317603439
5 0.0970290873783446
6 0.0975079373012679
7 0.0877286673642494
8 0.0843653461117515
9 0.0817675205893003
10 0.078804855296875
11 0.0789840859028228
12 0.0732090498399034
13 0.0738243450882698
14 0.0722315408702836
15 0.0783520494674634
16 0.0711730652671965
17 0.0679447150316952
18 0.0674496467046783
19 0.0653442230131038
20 0.0651314261047751
21 0.0681998897127756
22 0.065945956241662
23 0.0614035997847007
24 0.0607017258233904
25 0.0587107147365908
26 0.0598750331474149
27 0.0580230914124085
28 0.0567016823019668
29 0.0561501230862973
30 0.0609647665164068
31 0.0547418521309746
32 0.0556487075479519
33 0.0524372238864443
34 0.0507523461735551
35 0.051452076421624
36 0.050709755040665
37 0.0482318399385044
38 0.0524017656560094
39 0.0450930847822675
40 0.0458694548010867
41 0.043268126532094
42 0.0452593550237741
43 0.0434935743821032
44 0.0416642973586969
45 0.040591260684536
46 0.0407921751521574
47 0.0426440218357278
48 0.0416857415694092
49 0.0373629579747532
50 0.0386146013534134
51 0.040087258533704
52 0.0366892849656075
53 0.0387929491944272
54 0.0367053537142483
55 0.0367625231083655
56 0.0375422209386365
57 0.0353035452454
58 0.0406868167022707
59 0.0338514302983635
60 0.0344445815956578
61 0.0340078526043712
62 0.0342113567180355
63 0.0351949651585384
64 0.0343469425358112
65 0.0354167636401099
66 0.0349764034817244
67 0.0332934652226071
68 0.0319203562203705
69 0.0341473689001512
70 0.0309904710538307
71 0.0342775024057582
72 0.0353613799995705
73 0.0319026301387095
74 0.0322183768530846
75 0.0343751414656048
76 0.0319721885774649
77 0.0303433305407892
78 0.0308628422546855
79 0.0306172141758279
80 0.031625261958468
81 0.0305604371216814
82 0.0303755843244027
83 0.0297352440337895
84 0.0341301504336067
85 0.0291640961327841
86 0.030200938433472
87 0.0350676761177182
88 0.0285487129112798
89 0.0287114065897041
90 0.0292228449986385
91 0.0305184557336424
92 0.028409238074105
93 0.029158290916879
94 0.0316133865960591
95 0.0314023956650178
96 0.0292422092007953
97 0.0303767037067413
98 0.0270756350778247
99 0.0293249646213967
100 0.0278613524953251
101 0.0303655978564914
102 0.0282619892428735
103 0.0282434238772546
104 0.0270290639188411
105 0.0275017344872277
106 0.0263871128097406
107 0.0304835192749209
108 0.027513612883193
109 0.0281177001515749
110 0.0280629859158306
111 0.0280204210737631
112 0.0270514343754633
113 0.0275378408875626
114 0.0288588657475175
115 0.026473940274315
116 0.0267692539634692
};
\addplot [cedline, color3]
table {%
1 0.140873646669537
2 0.118449433073413
3 0.109919125674356
4 0.10765102181145
5 0.106466355351701
6 0.098583759063712
7 0.0989229106238476
8 0.0964352911295461
9 0.0925882659853441
10 0.0915961423615734
11 0.090950297947374
12 0.086907991195873
13 0.0865947552555839
14 0.08307385241294
15 0.0847937779853283
16 0.0804285813645484
17 0.0786791702476934
18 0.0819120474683961
19 0.0785409173522518
20 0.0777249831845994
21 0.0806884018843448
22 0.0744424409354181
23 0.0745261997703626
24 0.0786822166388204
25 0.07355367999755
26 0.0724387892568736
27 0.0711354343778543
28 0.0743758719208643
29 0.068983755560466
30 0.0717297811178856
31 0.0682255868670105
32 0.0683953095417356
33 0.0663831083834563
34 0.0655529321385129
35 0.068016551695206
36 0.067770409583954
37 0.0658651669237276
38 0.0666533015923834
39 0.0637505162818597
40 0.0659513495413429
41 0.0664555286006816
42 0.0658212215693963
43 0.063844024772195
44 0.0639682272048352
45 0.0642550598764993
46 0.0639289958285136
47 0.0626252766416513
48 0.0617394082974345
49 0.0606780032660339
50 0.0605531775418893
51 0.060926431753942
52 0.0603327958977611
53 0.0614268443294756
54 0.0613545934229947
55 0.06043657388742
56 0.0595695363949278
57 0.0590141990507143
58 0.0603905705405079
59 0.0588815579366602
60 0.0583756888261469
61 0.0585757091933032
62 0.0577912629751882
63 0.0588341971537798
64 0.0601469314899659
65 0.0622011829913183
66 0.0581845280135955
67 0.0595885955392006
68 0.0593709998888843
69 0.0560182032523391
70 0.0570845631180841
71 0.0565352543196151
72 0.0564990597792192
73 0.0567152409456773
74 0.0614434099998815
75 0.0547794380376398
76 0.0541054887036225
77 0.0581716611387855
78 0.0551532399195749
79 0.055119361478537
80 0.0567550784751372
81 0.0559588858919786
82 0.0556728881553334
83 0.0550966676586602
84 0.0543818176638646
85 0.0562992681204364
86 0.0533321800058273
87 0.0537033997307985
88 0.0537715745618943
89 0.0527593522749159
90 0.05284430023033
91 0.0528597151390371
92 0.052818105120201
93 0.0532455494215349
94 0.0537419573152633
95 0.0543079795353067
96 0.0538364063455159
97 0.0514210089991121
98 0.0506805153637095
99 0.0507860559815789
100 0.0540317378373529
101 0.0518659916704243
102 0.0514639725469233
103 0.0509171830535124
104 0.0522003268796993
105 0.0510861971171266
106 0.0499503921408184
107 0.0495638248883066
108 0.0500742783006225
109 0.0502820180218744
110 0.050114921724949
111 0.049048566082146
112 0.0492013431794684
113 0.0504334181736825
114 0.0509460200618292
115 0.0531289526337844
116 0.0502749931900124
117 0.0509679442719955
118 0.048424989195375
119 0.0488250929505594
120 0.0485772120334469
121 0.0485904194660272
122 0.047988221397874
123 0.048282381063492
124 0.0486958561564261
125 0.0477874803235558
126 0.0494595613081512
127 0.0480872229338867
128 0.0487102527063634
129 0.0477632109981834
130 0.0481415937873102
131 0.0488839691680911
132 0.0481482004027309
133 0.0482019181471878
134 0.0479276674877329
135 0.0487267056525074
136 0.0480289496934623
137 0.0471818713342305
138 0.0479115263810952
139 0.0484135119965088
140 0.0474558930578031
141 0.0472180794589689
142 0.0468381540863136
143 0.0471553106486726
144 0.0474607701377761
145 0.0477359073030816
146 0.0467222177470554
147 0.0472115751020254
148 0.0474479812997002
149 0.0479414251380565
150 0.0471011029788595
151 0.0479320006263639
152 0.0468964967575636
153 0.0461323502472568
154 0.0454953323206055
155 0.0465223071583798
156 0.0458483042780915
157 0.0456425729276591
158 0.0472463729193928
159 0.0471875086134712
160 0.0465611426195867
161 0.0449360330930582
162 0.0465636375836913
163 0.0460450936594377
164 0.0487924064951633
165 0.0464833617036537
166 0.0463074916114177
167 0.0467947744292838
168 0.0453916210929686
169 0.0462738546958763
170 0.0454934862461822
171 0.0449225599973633
172 0.0457007682515944
173 0.0449207128652558
174 0.0447821682323919
175 0.0441781067184548
176 0.0441041637441129
177 0.0447234847187583
178 0.0454042190515997
179 0.0446249104000274
180 0.0448425869186928
181 0.0448935487637661
182 0.0455793793935311
183 0.045468509610195
184 0.0448618201589484
185 0.0437332789970264
186 0.0441298269253003
187 0.0449187570745999
188 0.0441941994648671
189 0.0447832549316494
190 0.0443483722471965
191 0.0437580814476839
192 0.0438495623611144
193 0.0443564172828714
194 0.0440948117431705
195 0.045316030008119
};
\addplot [cedline, color4]
table {%
1 0.12648626030559
2 0.115983216008494
3 0.106271290325213
4 0.104609131831914
5 0.101546675986297
6 0.099896864187109
7 0.0952241697148866
8 0.0922784439457318
9 0.0904449878907441
10 0.0888625709397795
11 0.0864224346250657
12 0.0837241020902546
13 0.0826532440115257
14 0.0830898272404486
15 0.0847963034406027
16 0.0787484665196763
17 0.0779383431272533
18 0.0792528703638398
19 0.0757399197709221
20 0.0728566325594864
21 0.0742978482245114
22 0.0750177302502639
23 0.0751018153714722
24 0.0754403879990055
25 0.0746839378751323
26 0.0761837148854747
27 0.0696997463622215
28 0.0678294458361457
29 0.0678738492288464
30 0.0650787120324321
31 0.0725462629857663
32 0.0681126023145775
33 0.0680731655849529
34 0.0661768921755099
35 0.0700066855264685
36 0.0659880813256473
37 0.0637967700022968
38 0.0672228942908708
39 0.0638470711340036
40 0.0651855280809153
41 0.0651386784861372
42 0.0638923929341466
43 0.0685653805807758
44 0.0649850006380734
45 0.0624800987697554
46 0.0612867629099754
47 0.0642288536543145
48 0.0602893676326546
49 0.0635925743745511
50 0.0612332538517497
51 0.0607550487842083
52 0.0603283686476954
53 0.0622301328776094
54 0.0602386746667072
55 0.060437818413019
56 0.0599453064133617
57 0.0594522326435463
58 0.0597128891601935
59 0.0597260743837686
60 0.0592670412233258
61 0.0595849621994013
62 0.0595464639337859
63 0.0583119260270966
64 0.0580944656861282
65 0.0595288095373143
66 0.0592891681367065
67 0.0604333556471497
68 0.0571837496221408
69 0.0578265687727488
70 0.0584671650571835
71 0.0595142391078729
72 0.0578428683291936
73 0.0583307732028557
74 0.0590846883041738
75 0.058640582634208
76 0.057247389242399
77 0.0582626235427683
78 0.0566140106166046
79 0.058219069218086
80 0.0575458124934047
81 0.0569494100455386
82 0.0567394386425735
83 0.0567951082865497
84 0.0569485570259345
85 0.0570421715854339
86 0.0560122492943222
87 0.0552124347326333
88 0.0604277240332243
89 0.056380390979033
90 0.0554952349694731
91 0.0553142221268383
92 0.0546023477212885
93 0.0559548283159255
94 0.0562208795552495
95 0.0570406789391158
96 0.0546329143507183
97 0.054038942188368
98 0.055838802262556
99 0.0548772000593489
100 0.0551242034880979
101 0.0548931203723064
102 0.0547870157841772
103 0.0554743053661928
104 0.0547083650376918
105 0.0544352835151756
106 0.0559064768681345
107 0.0537661056422365
108 0.0543330858920366
109 0.0542428525307559
110 0.0541706813638114
111 0.0551059367250977
112 0.054629280604545
113 0.0546864571386056
114 0.0540964732811056
115 0.0534495390825973
116 0.0531866024686576
117 0.0548603178398626
118 0.0546022408433227
119 0.0534131579988737
120 0.0523355709378022
121 0.054214946963834
122 0.0549828677303486
123 0.0529243461033164
124 0.0547806042701238
125 0.0533577278032926
126 0.0531807158354729
127 0.0548817945380997
128 0.0523877372622663
129 0.0522622978290752
130 0.0528550775328211
131 0.052763318731206
132 0.0526031221602479
133 0.0519581141765206
134 0.0518551272059962
135 0.0512724777813469
136 0.0516163195197554
137 0.0541754929369922
138 0.0521897693041478
139 0.0520573402879425
140 0.0528556128570181
141 0.0528221010097472
142 0.051866808883708
143 0.0509291614029259
144 0.0538091056018102
145 0.0518407660574041
146 0.0526836519865794
147 0.052795975979204
148 0.0521891264872039
149 0.0523020416581412
150 0.0517567384873086
151 0.0512873832578391
152 0.0529049685167491
153 0.0514185204279893
};
\addplot [cedline, color5]
table {%
1 0.132327865445881
2 0.112699180284334
3 0.103930303314924
4 0.0969893475002577
5 0.0948160875012021
6 0.095311746779946
7 0.0875177383896439
8 0.0863085842950033
9 0.0819498995951786
10 0.079353073452193
11 0.0789752139202773
12 0.0736757180728438
13 0.0710906693641138
14 0.0667360865338429
15 0.0652747035045507
16 0.0650086133083936
17 0.0637483992944874
18 0.0646845124873483
19 0.0602128227337873
20 0.0599437797290208
21 0.0589123296027578
22 0.0567024248787347
23 0.0558613488887865
24 0.0525982118353236
25 0.0499975133628539
26 0.0492978332736211
27 0.0443977089206826
28 0.0433538912846931
29 0.040166748277525
30 0.0403522788035753
31 0.040179059942419
32 0.0376351726104753
33 0.0395317838876537
34 0.0309446999619176
35 0.0373125654788682
36 0.0275960079068092
37 0.0291803294663633
38 0.0267601164723619
39 0.0268664491228408
40 0.0285329472013436
41 0.0267245593148899
42 0.0273070073551009
43 0.0246269912098998
44 0.0250104645112599
45 0.0245395661533137
46 0.0228988741517282
47 0.0229735850626596
48 0.0228129607892598
49 0.0232938697707943
50 0.0220441788847106
51 0.0262253005160462
52 0.0241287874063503
53 0.0231238767518454
54 0.02390788671194
55 0.0222338785064682
56 0.0221106333151071
57 0.0221410300299569
58 0.0227977727561435
59 0.0214623198949064
60 0.0219145855900058
61 0.023053277938109
62 0.0205898405312361
63 0.0257147384457501
64 0.0200719457552099
65 0.0198612658860482
66 0.0208189178417193
67 0.0221489064002303
68 0.0210137366830279
69 0.0199693351946033
70 0.0194729205126867
71 0.0212439383036844
72 0.0207112735948531
73 0.0195835898425745
74 0.0206198390913075
75 0.0212550417213608
76 0.0243216342290049
77 0.0205011728596109
78 0.0205756186772017
79 0.0189827138984764
80 0.0135412895417957
81 0.0137492776624968
82 0.0130617115254359
83 0.0129743890279479
84 0.0128729510152756
85 0.0118261727983409
86 0.0113436406973428
87 0.0115834783892603
88 0.0117057857977048
89 0.0112606540016325
90 0.0114010544886447
91 0.0116067975461169
92 0.0109147271632788
93 0.0121134065060646
94 0.0123255008001957
95 0.0112374389229557
96 0.0139842890989932
97 0.0111398624094328
98 0.0133701899613667
99 0.0114434398991889
100 0.0111229257459922
101 0.0111178783404791
102 0.012211672371333
};
\end{axis}

\end{tikzpicture}


==> figures/07-stack-attention-cfls/train/marked-reversal.tex <==
% This file was created with tikzplotlib v0.9.17.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
\definecolor{color4}{rgb}{0.580392156862745,0.403921568627451,0.741176470588235}
\definecolor{color5}{rgb}{0.549019607843137,0.337254901960784,0.294117647058824}

\begin{axis}[
tick align=outside,
tick pos=left,
title={\MarkedReversal{}},
x grid style={white!69.0196078431373!black},
xmin=-4.5, xmax=116.5,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={Cross-entropy Diff.},
ymin=0, ymax=0.54925872805376,
ytick style={color=black}
]
\addplot [cedline, color0]
table {%
1 0.407937343357626
2 0.406673379731406
3 0.372391238237399
4 0.351812473359733
5 0.32357240979592
6 0.309122795606321
7 0.299000310758428
8 0.276547212845505
9 0.275656135257329
10 0.26609728692648
11 0.274600109564502
12 0.249067472234211
13 0.224473732535629
14 0.208065006328632
15 0.204548931942917
16 0.186096111484155
17 0.168703278401546
18 0.188194131525895
19 0.161302054323442
20 0.135856728944192
21 0.167427161283687
22 0.165666694854927
23 0.170259684057058
24 0.147085991565738
25 0.119632680188405
26 0.121160534607144
27 0.139647598604349
28 0.109199728556803
29 0.126825487946778
30 0.104455756165157
31 0.113849094225444
32 0.135601244862033
33 0.118275672154766
34 0.106184708584148
35 0.107727657950826
36 0.136723122293128
37 0.102416355056864
38 0.115738986962204
39 0.104742237698989
40 0.105482272113457
41 0.0888083542996947
42 0.107026100917816
43 0.0929357984919874
44 0.0922830646266051
45 0.0985687006906649
46 0.0970681893972969
47 0.104433672315068
48 0.0870433622866147
49 0.111457475351803
50 0.0801498749103032
51 0.0880567397135852
52 0.0823622577914133
53 0.0857751452357638
54 0.085086779767956
55 0.0926028780382855
56 0.0955975656001535
57 0.0785746813130537
58 0.0777776056485756
59 0.0815685340535838
60 0.0790221172931633
61 0.0762408029266535
62 0.110289266575796
63 0.0752784217310498
64 0.0715894503435694
65 0.0909076979595895
66 0.0814300954923098
67 0.0924613547526794
68 0.0751390152430166
69 0.0954295580537652
70 0.0815491289191114
71 0.0812346987169965
72 0.0683978483071449
73 0.0774867009001435
74 0.0806814027808829
75 0.068794089265296
76 0.0935285409756605
77 0.0706405633606909
78 0.0825288676069451
79 0.0689562049758167
80 0.0732443098901343
81 0.0726196766364679
82 0.0653049145680843
83 0.0670787411126744
84 0.0704783901446623
85 0.0799704240157237
86 0.0896352160821527
87 0.108570507008069
88 0.0649710990609826
89 0.0711003350158372
90 0.0684137292463137
91 0.076434098272245
92 0.061324360511638
93 0.0656230613115117
94 0.0652644415967835
95 0.0691424650678349
96 0.0669970260339052
97 0.0889042519222029
98 0.0639506149942913
99 0.0616994870336699
100 0.0797249761318947
101 0.0551061662627121
102 0.0619329227109435
103 0.0919627361440399
104 0.0669309390683655
105 0.0604859773023896
106 0.0605221928831618
107 0.0755251035046117
108 0.0841822223434318
109 0.0605107207822168
110 0.0783523518827183
111 0.0584732989044406
};
\addplot [cedline, color1]
table {%
1 0.450644551811041
2 0.41355275055666
3 0.424018519224028
4 0.379640270887246
5 0.523088179906435
6 0.377357102323847
7 0.356010365645214
8 0.350916098582356
9 0.339762240395076
10 0.383049195327853
11 0.367778360008674
12 0.338451258402933
13 0.331998721897044
14 0.326382179132665
15 0.32367172304894
16 0.298598167696247
17 0.27338463933869
18 0.153186051328047
19 0.0208621652235936
20 0.00666169770889458
21 0.00432093486097457
22 0.00393423527569803
23 0.00799161707147145
24 0.00502315750136406
25 0.00392592160289179
26 0.00463500897225222
27 0.00398247972982346
28 0.00314966103950931
29 0.00430884643795887
30 0.00478735767371447
31 0.00341562188082078
32 0.00298389111356268
33 0.00428525474232244
34 0.00274603795791495
35 0.00304054738202719
36 0.00365789535083072
37 0.00539374757323635
38 0.00444855041666203
39 0.00317494284083797
40 0.00484482817167931
41 0.00241901730167693
42 0.00402709639945192
43 0.00361992641381931
44 0.00248727177866676
45 0.00298806681385327
46 0.00386109714781313
47 0.00245871407215564
48 0.00407278942031253
49 0.00314446471659541
50 0.0055635980169822
51 0.00450838346242916
};
\addplot [cedline, color2]
table {%
1 0.429171558091922
2 0.368746003163695
3 0.359065958433296
4 0.343954564498419
5 0.315360457308657
6 0.328131042776405
7 0.273653492335847
8 0.287752224848584
9 0.261870259729485
10 0.23379905762786
11 0.00957485352507831
12 0.00680687363270827
13 0.00585569791761353
14 0.00484446053059767
15 0.00455258387102658
16 0.00574218680035649
17 0.00619505917698249
18 0.00457789827319416
19 0.00526893246068377
20 0.0040556814560011
21 0.00297484793967068
22 0.00767981859281353
23 0.00419853704308293
24 0.00509206765379855
25 0.00716284558750097
26 0.0026331455431915
27 0.00365777043501869
28 0.00309109512441397
29 0.00495279615511973
30 0.00627250210301611
31 0.00573344423551131
32 0.00375893737478589
33 0.00559348243409158
34 0.00221102770291598
35 0.00757592980813326
36 0.00254866676107607
37 0.00183527240301645
38 0.00393621362039065
39 0.00401610003526531
40 0.00265937552349765
41 0.00349593558615513
42 0.00493540271023052
43 0.00768354820861544
44 0.00687966958697955
45 0.00343935107936466
46 0.00681385513824317
47 0.00485977544802862
};
\addplot [cedline, color3]
table {%
1 0.353067452306438
2 0.252733318266728
3 0.26328963927605
4 0.16713183426606
5 0.144307782174045
6 0.112724313157581
7 0.0834986763862972
8 0.0894171603321129
9 0.108422440500322
10 0.0948414225833796
11 0.0665680113027629
12 0.0557641572403197
13 0.0467504904702091
14 0.0670798512716675
15 0.0494800903500655
16 0.0311653592583093
17 0.0305655288922496
18 0.0296788410370706
19 0.0327075760017026
20 0.0299491312891343
21 0.0415235691511104
22 0.0384635767520374
23 0.0318470515122148
24 0.02067498970362
25 0.0246340456647737
26 0.0344556214588834
27 0.0152891717575118
28 0.0303150673359043
29 0.0168731076080121
30 0.0177072647022009
31 0.0428197950757808
32 0.0162374414201067
33 0.0260573098887253
34 0.0197400613734671
35 0.0146712713875211
36 0.0103159084395584
37 0.0180243630085174
38 0.0161383712359792
39 0.0118222552151947
40 0.027835773591488
41 0.0102309344590777
42 0.00978299662898546
43 0.00762565661988673
44 0.0102008427914301
45 0.0121056642156078
46 0.0102087068346413
47 0.0100799855329339
48 0.0141838375030697
49 0.00697071919498704
50 0.011922074331183
51 0.00838419747849284
52 0.00558184418104657
53 0.00698979876359135
54 0.00846739928669699
55 0.00884851173780593
56 0.00517222509364962
57 0.0110717707392182
58 0.00565681533532547
59 0.00698215087896198
60 0.012484031796655
61 0.00643779329281335
62 0.0106741801107041
63 0.00982530286812244
64 0.0110331252585018
65 0.00909958723608062
66 0.00558394022517439
};
\addplot [cedline, color4]
table {%
1 0.306691262321371
2 0.00606139635165504
3 0.00224859873032768
4 0.00393667722517643
5 0.00128532797504172
6 0.00229213002452072
7 0.00127698566866691
8 0.00247966512216669
9 0.00191404037943005
10 0.00106451687649955
11 0.00268099562709151
12 0.000106267047204345
13 0.00198761397144864
14 0.000265917519227887
15 0.0010552816010525
16 -0.000109046045016215
17 9.41037012526236e-05
18 0.000557017392007142
19 0.000171460059898709
20 0.000811001907124631
21 0.000628826830213425
22 0.000201541472284128
23 -0.000219680668526456
24 -1.76438266523693e-05
25 0.000523380272250851
26 0.000235513731383807
27 0.000137323452734428
28 0.000207622510387084
29 0.00187753486088027
30 -0.000322783040065611
31 0.000283186459090146
32 9.93745026629522e-05
33 1.35786192881904e-05
34 0.001678876154588
35 0.000259188227174911
36 0.000242729647359441
37 0.000269565911650949
38 0.000108618610355271
39 -9.655580808271e-05
40 -0.0001703640164325
};
\addplot [cedline, color5]
table {%
1 0.00395678862812576
2 0.0168384329995852
3 0.00152072297873923
4 0.00219468091081998
5 0.00193606252884099
6 0.00178950133409195
7 0.00302001305582628
8 0.00401438281384686
9 0.00424957856484354
10 0.00209702811521634
11 0.000596109041785253
12 0.00198728903072082
13 0.00203640564890079
14 0.00337556504593528
15 0.0038183710578531
16 0.000368170755576158
17 0.000727669423990329
18 0.00106594604295857
19 0.000403809833040891
20 0.00149298969764866
21 0.000200187250203265
22 0.000410141928043783
23 0.000194016221607252
24 0.00105434478218536
25 0.004403461113625
26 0.00178115123875289
27 0.00206987813348825
28 0.000385625132170164
29 0.000129705341491537
30 0.00111218749326747
31 0.000481659345426877
32 0.000270095849001561
33 0.000654059424424147
34 9.38940814449452e-05
35 0.000543512510092325
36 -6.80658412538504e-06
37 0.00028698360453483
38 0.000514615707229327
39 0.00212596026951917
40 0.000505280887413806
41 0.000619646717041566
42 0.000607715619858173
43 3.68857565086755e-05
44 0.000293397629262671
45 0.000495215418846284
46 0.000629142794694892
};
\end{axis}

\end{tikzpicture}


==> figures/07-stack-attention-cfls/train/padded-reversal.tex <==
% This file was created with tikzplotlib v0.9.17.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
\definecolor{color4}{rgb}{0.580392156862745,0.403921568627451,0.741176470588235}
\definecolor{color5}{rgb}{0.549019607843137,0.337254901960784,0.294117647058824}

\begin{axis}[
tick align=outside,
tick pos=left,
title={\PaddedReversal{}},
x grid style={white!69.0196078431373!black},
xmin=-7.45, xmax=178.45,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={Cross-entropy Diff.},
ymin=0, ymax=0.287646507702059,
ytick style={color=black}
]
\addplot [cedline, color0]
table {%
1 0.256841616446029
2 0.258488082432297
3 0.237930255069003
4 0.223185916168592
5 0.214112635812542
6 0.209803335979911
7 0.220403918312773
8 0.210589257540302
9 0.204788907729961
10 0.205983303341993
11 0.207970452573123
12 0.204795543564346
13 0.196254859931605
14 0.193873681094272
15 0.195187801465469
16 0.181541599612876
17 0.186979553309907
18 0.179987890868621
19 0.193615977383269
20 0.171530141584837
21 0.182664602826061
22 0.171143416448027
23 0.168425043249493
24 0.175143746236888
25 0.161459181894887
26 0.158162965386139
27 0.203445941622008
28 0.155226360534585
29 0.15898331301867
30 0.159916180703143
31 0.163111796581682
32 0.152107217310184
33 0.150613879402581
34 0.153106811417764
35 0.156592645605786
36 0.149517002962757
37 0.14586672340123
38 0.145198413317374
39 0.154677509177437
40 0.145617202980579
41 0.146298140213734
42 0.144830019289108
43 0.151630806235452
44 0.137516924401951
45 0.151611143187693
46 0.149036226087265
47 0.136723122645438
48 0.143931687339008
49 0.150736831074516
50 0.142513424526682
51 0.138597587331275
52 0.136119877297229
53 0.142597824973397
54 0.132449043428446
55 0.143258193937669
56 0.133077122068737
57 0.142947479452067
58 0.137188037970354
59 0.132670845196412
60 0.132815669914735
61 0.132346875795993
62 0.137967739752844
63 0.134076286031282
64 0.137035122869961
65 0.138585667021073
66 0.134584074466514
67 0.129963423878862
68 0.137133122829833
69 0.132835660933804
70 0.130678256515407
71 0.129294354536345
72 0.133609738719095
73 0.130099852201636
74 0.128012047889952
75 0.133726261696419
76 0.127779307821858
77 0.141358316044535
78 0.141681908988721
79 0.126494670472225
80 0.126870718264408
81 0.130705413402991
82 0.12906648479144
83 0.124990734293574
84 0.124960479194036
85 0.129217949532636
86 0.134366263439237
87 0.134057906183967
88 0.151806633381127
89 0.1325050642029
90 0.129937193154843
91 0.125413535893757
92 0.126883768577928
93 0.129744987370696
94 0.124525880653665
95 0.128173188800196
96 0.12731886580223
97 0.124284350472141
98 0.121838764237943
99 0.131337826366919
100 0.126394896624182
101 0.132989045271787
102 0.124870255479627
103 0.126822818714526
104 0.12465408684738
105 0.121547229347035
106 0.122157221841874
107 0.122711239254856
108 0.116659904449192
109 0.122929209063909
110 0.1171505683143
111 0.120265845691111
112 0.125251425158133
113 0.118171397675762
114 0.124966720802845
115 0.128137321888151
116 0.114060115217974
117 0.134695687266549
118 0.114293246211625
119 0.118694719944108
120 0.11901441848283
121 0.116629485744771
122 0.124117786612126
123 0.111216316601051
124 0.129520210760789
125 0.113104946626709
126 0.120874577958728
127 0.109561502577233
128 0.110924507173786
129 0.116729810315536
130 0.10879384917114
131 0.115864411178107
132 0.11330886063125
133 0.11984319195725
134 0.112629449023153
135 0.111087287940582
136 0.109459380002759
137 0.111645275913356
138 0.126368210370351
139 0.117856842219651
140 0.123207848361508
};
\addplot [cedline, color1]
table {%
1 0.27401993627965
2 0.272914923172548
3 0.250598261207529
4 0.243346885138454
5 0.23322434286388
6 0.235466991768299
7 0.237890739622261
8 0.234768129215897
9 0.224570172115879
10 0.22019648401742
11 0.219603113281644
12 0.217648397957911
13 0.212269511262166
14 0.216462238800571
15 0.207056299891925
16 0.201902899226226
17 0.200370712686275
18 0.198051257615708
19 0.198545467276266
20 0.198367991358399
21 0.196747916966372
22 0.195053415474991
23 0.192746440876872
24 0.196450961366691
25 0.187664524672441
26 0.190143949262196
27 0.186225360260265
28 0.182649934312311
29 0.184973499473662
30 0.189510416561731
31 0.18703845858555
32 0.180955996648975
33 0.178958979073397
34 0.194700949771757
35 0.181759999267356
36 0.176872251474686
37 0.179169462553174
38 0.17891162496334
39 0.176619123235499
40 0.17428305064271
41 0.177197220804084
42 0.166924941873153
43 0.168354357143826
44 0.170365995992511
45 0.164530123841106
46 0.168260061011149
47 0.165979039192051
48 0.165113958026282
49 0.165176840001811
50 0.160644551644168
51 0.170015108032148
52 0.1616015139305
53 0.158803757058248
54 0.154252470057571
55 0.155311380208563
56 0.150140193540933
57 0.158740004949182
58 0.152775408235973
59 0.155972358189157
60 0.155046957949297
61 0.146712770144317
62 0.155402974793563
63 0.154760824972476
64 0.154981429884587
65 0.150110218737166
66 0.149540035814916
67 0.14841495802924
68 0.148166862648596
69 0.143544505071355
70 0.143550321281158
71 0.147816010633554
72 0.13966362502266
73 0.150056202675235
74 0.141974926410502
75 0.140738132875747
76 0.14193763134197
77 0.140020215451558
78 0.141253512020017
79 0.141555484559598
80 0.138530611023456
81 0.138160028107828
82 0.140423203074701
83 0.145585391858052
84 0.136009832624845
85 0.147567384802663
86 0.141589933272156
87 0.138424435475461
88 0.137515261467321
89 0.133088366846927
90 0.138655174144016
91 0.135439826091423
92 0.14006587165867
93 0.135779393072716
94 0.139229664342816
95 0.136534126465649
96 0.132038403486507
97 0.130104518219948
98 0.131874405267012
99 0.137198490238795
100 0.135300511781093
101 0.131904753131868
102 0.136404752320531
103 0.13702199896599
104 0.131516519266018
105 0.125238448537292
106 0.126655935609711
107 0.127051597576291
108 0.133194735986155
109 0.138596846440747
110 0.128137039482735
111 0.126944253291835
112 0.128473640718236
113 0.12806570624857
114 0.122930559130736
115 0.121306172070361
116 0.124624012559238
117 0.127281521056301
118 0.123583749814136
119 0.123915267996019
120 0.128878536010951
121 0.123700019835474
122 0.124361200393632
123 0.122255817429709
124 0.120491708849861
125 0.124084957386948
126 0.122286454140901
127 0.12158717885918
128 0.121014811616755
129 0.117960132604986
130 0.12127415095078
131 0.124879609471769
132 0.123564302368086
133 0.120444841028655
134 0.119696876139799
135 0.117355318932799
136 0.117080603088783
137 0.119780992300619
138 0.123180618409706
139 0.118469580899551
140 0.119539934500459
141 0.124910129103912
142 0.117840332496304
143 0.123709874245419
144 0.119936083911276
145 0.115251727714788
146 0.123116774254942
147 0.115937326956986
148 0.116214850259003
149 0.117839095720485
150 0.116889218385436
151 0.114767146907281
152 0.115087594443584
153 0.11457968820332
154 0.115521312235754
155 0.114835124517289
156 0.117717546230022
157 0.113281485809345
158 0.116776726730913
159 0.114821594184696
160 0.111542394916649
161 0.116934041046213
162 0.113553176597788
163 0.114763147990241
164 0.118140610085591
165 0.117849926687795
166 0.121557155529228
167 0.112011522188476
168 0.113465742427023
169 0.113583838727456
170 0.112288180748754
};
\addplot [cedline, color2]
table {%
1 0.267272871002358
2 0.257477295901889
3 0.236866500572353
4 0.232976775443109
5 0.21899397204436
6 0.222747020511735
7 0.217342911397927
8 0.214458298714417
9 0.216416094907599
10 0.211951939968902
11 0.213187962043945
12 0.206331992410812
13 0.182310147335129
14 0.15452119453929
15 0.129640786710509
16 0.121701555272583
17 0.0970217548467394
18 0.0910688835443658
19 0.0869500717862955
20 0.0811608616782608
21 0.0751902416589024
22 0.0958735813085656
23 0.0647740259949592
24 0.0609954896529733
25 0.0634926835484046
26 0.0552129129683007
27 0.0491876282266263
28 0.0477056707649281
29 0.0367010153953116
30 0.0352220863636989
31 0.0390588059859103
32 0.0240626861481448
33 0.0266321584276151
34 0.0267646439563702
35 0.0286427882393149
36 0.0165733338558946
37 0.0158329152360505
38 0.0133381673141925
39 0.0256696421659794
40 0.0198538205235534
41 0.0145414119682435
42 0.0130746695868141
43 0.0139493932981255
44 0.0105645037562394
45 0.0106998502465547
46 0.0097780192598369
47 0.0101235200867876
48 0.00771494208766893
49 0.00842704305682951
50 0.00935519315648159
51 0.00958113668102661
52 0.00921057377187312
53 0.00831823566217366
54 0.0114141256054344
55 0.00782195570288952
56 0.00586670026751929
57 0.00968421331258074
58 0.00761416237779
59 0.0104725755682358
60 0.00594920675488653
61 0.0139498429093706
62 0.00669507203067193
63 0.0105947399283092
64 0.00694612846730946
65 0.00778814670525052
66 0.00617135915544809
};
\addplot [cedline, color3]
table {%
1 0.244501256489311
2 0.2110931681642
3 0.198494152917685
4 0.190063985459929
5 0.170850776474001
6 0.162905135908219
7 0.15397966558093
8 0.148627412058445
9 0.147955950078912
10 0.141064448414233
11 0.136785960558568
12 0.125099786600653
13 0.124237944790247
14 0.118245451403751
15 0.1133415886386
16 0.105551602202404
17 0.10493658894852
18 0.101354507340224
19 0.0986315334571245
20 0.108663893030735
21 0.0920297883822911
22 0.106895816520354
23 0.0839033264398775
24 0.0859210374822338
25 0.0946524666067878
26 0.104107147506261
27 0.0763216654901101
28 0.0775771106263761
29 0.0816530329618436
30 0.0907590897210916
31 0.0731834377303673
32 0.0759605748477328
33 0.0807947608693994
34 0.0761609556523404
35 0.0809888144831406
36 0.0651892863971382
37 0.113234058541302
38 0.0637027146052027
39 0.075242106426359
40 0.0637735383661645
41 0.0607641585000415
42 0.0703657344150396
43 0.0639622144329535
44 0.0607084722750844
45 0.0785383357270334
46 0.060619955823011
47 0.0610932318024762
48 0.0553787247294104
49 0.0600072300511396
50 0.0631903547682161
51 0.0679390714080136
52 0.0616773946101378
53 0.056599724248945
54 0.0570065569285729
55 0.0523548055620366
56 0.0586074417573092
57 0.0600961275683755
58 0.0553788068193917
59 0.0519165858995833
60 0.053744044941708
61 0.0514204024725914
62 0.0523895518450112
63 0.0527140666439062
64 0.0553104235296306
65 0.0527990059432228
66 0.05160384269924
67 0.0553568064632806
68 0.0508759818960732
69 0.0515912353508614
70 0.054124999707403
71 0.0502013928661928
72 0.0477213519976939
73 0.0552666656218492
74 0.0466458973439935
75 0.0473765114557231
76 0.0512304165437543
77 0.0476435085152532
78 0.0446571435220225
79 0.0455706112286408
80 0.0514471047598911
81 0.0471155681711712
82 0.0472102538466649
83 0.0451192066928676
84 0.0434832733409249
85 0.0440650256442186
86 0.0480001655868942
87 0.0445530046576071
88 0.0421574745346935
89 0.0452782662943614
90 0.0536992317021099
91 0.0421185443559641
92 0.0456409071895865
93 0.0405407637570354
94 0.0432228077208102
95 0.0456662722075311
96 0.0474125895963457
97 0.0472762967636606
98 0.047916802598177
99 0.0425585833902266
100 0.0411489603363825
101 0.0403090320145286
102 0.0423297307037471
103 0.0444827151665334
104 0.0438728066119083
105 0.0422937182264595
106 0.0396848140901931
107 0.0425989930678676
108 0.0397728684271137
109 0.0392964820290439
110 0.0402646960542823
111 0.03984173885868
112 0.0482101962728187
113 0.0425871031470823
114 0.0386201273736296
115 0.0407068009808296
116 0.0378372213897053
117 0.0425172574013832
118 0.0435649300907999
119 0.0426576091423659
120 0.0413299652304198
121 0.0377670430841467
122 0.0397631127887612
123 0.0425052833551283
124 0.0393381081661932
125 0.038069860664098
126 0.0402484445990995
127 0.037274988279973
128 0.0396838968167118
129 0.0422854010727625
130 0.0384964063768415
131 0.0405100192692635
132 0.0395195245027939
133 0.0355624424919402
134 0.0415439816412425
135 0.0388821282614576
136 0.036864729703048
137 0.037963947590567
138 0.0401580983612505
139 0.0362912394572414
140 0.0348427502599624
141 0.0367683902670276
142 0.0355579209036168
143 0.0352137177831954
144 0.0358927143463497
145 0.0360838789275834
146 0.0361189441201821
147 0.0336489902676662
148 0.0443753212086268
149 0.0345400433691836
150 0.0377343750739669
151 0.033577342822731
152 0.0416486007671706
153 0.034977815795021
154 0.0341098777269832
155 0.0346979451068582
156 0.0350852184160497
157 0.0362204505025981
158 0.0388158624611294
159 0.0356931410508042
160 0.0350759195812816
161 0.0362601130164486
};
\addplot [cedline, color4]
table {%
1 0.228845027739082
2 0.210357459783586
3 0.198497524364069
4 0.185261783979203
5 0.176579937899276
6 0.172653003937873
7 0.165039773743573
8 0.155070813351657
9 0.148027475756311
10 0.144125075661287
11 0.138107970210467
12 0.132375807843005
13 0.13803325646125
14 0.129799613836982
15 0.125374962733302
16 0.126428958233931
17 0.119175160399159
18 0.116110174696041
19 0.113274827881499
20 0.110571939134919
21 0.109103516460613
22 0.103751442490718
23 0.100732252241417
24 0.124211801205808
25 0.0958900175351195
26 0.105638835929266
27 0.103286152905441
28 0.0986963643902557
29 0.0930260599224015
30 0.0968319929150621
31 0.0847766713964882
32 0.0937766129293095
33 0.0818102314489473
34 0.0859293825525554
35 0.0820704163633388
36 0.0843898077675265
37 0.0887135379631985
38 0.0816053658708471
39 0.0776898836586858
40 0.0795796322918242
41 0.0796974883560104
42 0.0755829996613348
43 0.0797663909889925
44 0.0990709990074214
45 0.07808814441868
46 0.0838640563080297
47 0.0725947493373619
48 0.0795329172030297
49 0.068768559085523
50 0.0757149553327582
51 0.075882079534042
52 0.071921709804971
53 0.0723104500204637
54 0.0697220647471246
55 0.068836362399436
56 0.0642336394785634
57 0.069348048415988
58 0.0635057732644601
59 0.0628396599629084
60 0.0665457796114827
61 0.0691239103602081
62 0.0620829054093973
63 0.0708705824635865
64 0.0717653505057907
65 0.067679201542805
66 0.067708373148007
67 0.0757026102792125
68 0.0675701843280384
69 0.061734391308889
70 0.0662001125470775
71 0.0631889255588293
72 0.0589035014552823
73 0.0586984545532445
74 0.0653295898603365
75 0.0551838710404198
76 0.0586487151712877
77 0.0580447958931203
78 0.0591422486214976
79 0.0565004685710069
80 0.0586820652924826
81 0.0564916430572966
82 0.0626125150392075
83 0.0545211142895008
84 0.052984452340095
85 0.0580103637894721
86 0.0512541228897811
87 0.0598161226120354
88 0.0562145803872996
89 0.0562998323287026
90 0.0608183125593258
91 0.0530898234500664
92 0.0567312117693961
93 0.0518270997426814
94 0.0502408990329405
95 0.0504140614276319
96 0.0523165431286018
97 0.0513623049042776
98 0.0490178776114915
99 0.0518527146608111
100 0.050037769121042
101 0.049132393628114
102 0.0492423693479566
103 0.0474691010036759
104 0.0533941483087052
105 0.0518547671098323
106 0.0493901096034078
107 0.0505432148011418
108 0.0470925235864643
109 0.0464346162040607
110 0.0520978293804056
111 0.0527476753438381
112 0.0501252762958225
113 0.0456462573175102
114 0.0541567670654359
115 0.0475506493537502
116 0.0461370005572373
117 0.0485208858834825
118 0.0500563568118459
119 0.0524675220838172
120 0.0439199713325353
121 0.0475598839347827
122 0.049088268232954
123 0.0457761930961291
124 0.0535387357470628
125 0.0489884026397746
126 0.0460375003988839
127 0.0443415033947594
128 0.0425168392464427
129 0.0478305347122269
130 0.0426257219902761
131 0.0470429460002746
132 0.0474799854956333
133 0.0425289379145618
134 0.0447496286067871
135 0.0429694451868859
136 0.0430048960523215
137 0.0475587296168172
138 0.0437918631892256
};
\addplot [cedline, color5]
table {%
1 0.234167041733384
2 0.213385491518005
3 0.183040351517694
4 0.156623867261029
5 0.143270226194886
6 0.116068469303771
7 0.10530340136508
8 0.114459825971759
9 0.084705140259055
10 0.0745205120112653
11 0.06699105462044
12 0.0759018095103378
13 0.0409953649793276
14 0.0317660274498098
15 0.0102332715518524
16 0.0038762773832432
17 0.00498385302492244
18 0.00482762006450971
19 0.00548426662202534
20 0.0082242799439296
21 0.00444206122982493
22 0.00333756585605
23 0.00271505475640582
24 0.00364593777076799
25 0.00496411158564525
26 0.00355257179949875
27 0.00322122768336547
28 0.00258776474598993
29 0.00252754047438236
30 0.00610428849763717
31 0.00599697989836345
32 0.00287786983895777
33 0.00255007145866304
34 0.00343112308825705
35 0.00310932823898313
36 0.00226612681276611
37 0.00305290288288584
38 0.0032254225988283
39 0.00422382547688011
40 0.00250269583476626
41 0.00192929854734203
42 0.00318450001895015
43 0.00339945327600505
44 0.004600833724692
45 0.00271753872059682
46 0.00148850783146609
47 0.00179119187810922
48 0.00427248796613683
49 0.00253593610961156
50 0.00385232179758227
51 0.00159853079018707
52 0.00223716232656623
53 0.00274863057798019
54 0.00268182043507925
55 0.00241513497691548
56 0.00161379412603402
};
\end{axis}

\end{tikzpicture}

